Evaluating the Impact of Source Code Parsers on ML4SE Models

As researchers and practitioners apply Machine Learning to increasingly more software engineering problems, the approaches they use become more sophisticated. A lot of modern approaches utilize internal code structure in the form of an abstract syntax tree (AST) or its extensions: path-based representation, complex graph combining AST with additional edges. Even though the process of extracting ASTs from code can be done with different parsers, the impact of choosing a parser on the final model quality remains unstudied. Moreover, researchers often omit the exact details of extracting particular code representations. In this work, we evaluate two models, namely Code2Seq and TreeLSTM, in the method name prediction task backed by eight different parsers for the Java language. To unify the process of data preparation with different parsers, we develop SuperParser, a multi-language parser-agnostic library based on PathMiner. SuperParser facilitates the end-to-end creation of datasets suitable for training and evaluation of ML models that work with structural information from source code. Our results demonstrate that trees built by different parsers vary in their structure and content. We then analyze how this diversity affects the models' quality and show that the quality gap between the most and least suitable parsers for both models turns out to be significant. Finally, we discuss other features of the parsers that researchers and practitioners should take into account when selecting a parser along with the impact on the models' quality. The code of SuperParser is publicly available at https://doi.org/10.5281/zenodo.6366591. We also publish Java-norm, the dataset we use to evaluate the models: https://doi.org/10.5281/zenodo.6366599.

==> FSE’22_ Parsers evaluation/sections/01-introduction.tex <==
\section{Introduction}\label{sec:introduction}

The field of applying machine learning (ML) algorithms to source code rapidly grows~\cite{sharma2021survey}.
Earlier ML models represented code as a set of explicitly defined metrics or as plain text. The latter makes it possible to reuse approaches from the Natural Language Processing (NLP) domain~\cite{Ernst2017nlp_for_se}.
While any file with source code can indeed be seen as a text document, source code has a richer underlying structure compared to natural languages. Nowadays, there are increasingly more works that take this underlying code structure into account~\cite{alon2018code2seq, allamanis2020typilus, zugner2021codetrans}.

Every programming language has its own strict syntax that can be represented as a set of predefined rules determining all possible language constructions.
Parsing the raw source code with these rules allows representing it in the form of a parse tree, and then as an abstract syntax tree (AST).
By working with this structure and also with its possible extensions (\eg path-based representation~\cite{alon2018general}, graph-based representation~\cite{allamanis2017learning}) researchers improve results for various software engineering tasks: code summarization~\cite{alon2018code2seq}, type inference~\cite{allamanis2020typilus}, bug detection and repair~\cite{Hellendoorn2020Global}, malware detection~\cite{rusak2018ast}.

Aside from the ML domain, the representation of code as an AST is crucial for its analysis and execution: it is used by compilers, static analysis tools, and integrated development environments (IDEs).
As a result, there exist a lot of different parsers for building ASTs from source code. Most parsers are tailored for a specific problem and have their own features. For example, \textsc{Tree-sitter}~\cite{max_brunsfeld_2022_6326492} aims to work with incremental parsing, \textsc{ANTLR}~\cite{10.5555/2501720} makes it easier to create new languages by providing parser generators, and so on.
All the parsers have different use-cases and require different levels of information from code, therefore, they might build different ASTs.

Even though for most languages there are many available parsers, not all the research works that use information from ASTs to train ML models provide enough details on how they build syntax trees.
Machine learning models are very sensitive to the input data, and as different parsers build ASTs in a different manner, the choice of a parser might affect the model's quality. In turn, it might lead to unreproducible results or even incorrect model comparison if the models use different parsers.

In this work, we investigate whether the selection of a source code parser affects the final quality of ML models.
We studied the impact of the parser choice on two popular models that work with ASTs in a different manner: TreeLSTM~\cite{DBLP:journals/corr/TaiSM15} and Code2Seq~\cite{alon2018code2seq}.
TreeLSTM is an extension of the regular LSTM~\cite{hochreiter1997lstm} network that was adapted to work with tree-structured data.
Although it falls behind in quality compared to modern models, it is useful to study since it utilizes trees without further modifications.
On the other hand, Code2Seq is a popular approach that was reused in various tasks apart from the original method name prediction~\cite{nagar2021code, Zhang2020CBPath2Vec}.
Code2Seq employs path-based representation~\cite{alon2018general} to work with code, which also relies on the information from the code's AST.

As a comparison benchmark, we use the method name prediction task for the Java programming language.
In addition to its practical applicability, method name prediction suits as a popular benchmark in the ML for SE domain~\cite{alon2018code2seq, fernandes2018structured, zugner2021codetrans}, as it allows evaluating how good models are in code understanding. We compare both models backed by eight different Java parsers. In order to do so, we develop \toolname, a tool based on PathMiner~\cite{kovalenko2019pathminer}. \toolname supports mining code representations suitable for ML models from five programming languages and twelve language-parser pairs in a unified manner.

Our results suggest that parsers can significantly affect the final quality of model predictions.
Proper parser choice for the Code2Seq model may increase the quality of the model by up to $5.5\%$ in terms of F1-score compared to the least suitable parser.
For a simpler TreeLSTM model, the parser selection is even more crucial, with the difference between the most and least suitable parsers being about $27.0\%$. Notably, for TreeLSTM and Code2Seq, the relative ordering of parser is different, meaning there are no universally good or bad parsers. Therefore, when choosing a parser, researchers and practitioners should take into account the model's properties and characteristics of trees produced by different parsers. 

With this work, we make the following contributions:
\begin{itemize}
    \item We investigate the impact of the parser selection step on the quality of machine learning models working with structural representations of code.
    To the best of our knowledge, this work is the first to study this part of the data preprocessing pipeline. We show that depending on the specific parser used, results of both TreeLSTM and Code2Seq can vary significantly.
    
    \item We present \toolname, a tool based on PathMiner, that allows running multiple parsers for different programming languages in the same manner. \toolname allows running experiments with different parsers by changing a single field in a YAML configuration file. Our tool separates the parsing step, allowing further data processing steps (\eg filtering, storage) to be parser-agnostic. It makes support of new languages, parsers, and mining tasks easy for the users.

    \item We publish a dataset of open-source Java projects called \javanorm. It is comparable in size to the commonly used \textit{Java-small} dataset, but its validation and testing parts include more diverse projects making evaluation more robust and representative.

\end{itemize}


==> FSE’22_ Parsers evaluation/sections/02-background.tex <==
\section{Background}\label{sec:background}
\newdimen\figrasterwd
\figrasterwd\textwidth

\begin{figure*}[ht]
    \centering
\parbox{\figrasterwd}{
    \parbox{.4\figrasterwd}{
        \centering
        \subcaptionbox{
Examples of rules that define syntax for method declaration.
\label{fig:rules}
        }
        {\includegraphics[width=\hsize]{figures/grammar-rules.png}}
        \vskip3em
        \subcaptionbox{
Java method code snippet example.\label{fig:java_method}
        }
        {\includegraphics[width=\hsize]{figures/java-method.png}}  
    }
    \hskip1em
    \parbox{.6\figrasterwd}{%
        \subcaptionbox{
An example of a parse tree built for the code snippet on the left. Blue nodes are intermediate abstraction nodes. Green nodes contain actual code tokens.
\label{fig:ast}
        }
        {\includegraphics[width=\hsize]{figures/ast.pdf}}
        }
    }
\caption{
An example of a code snippet, its correposnding parse tree, and a subset of grammar rules.
}
\vspace{-0.5cm}
\end{figure*}


In our work, we analyze the impact of choosing a parser on the quality of ML4SE models.
In this section, we first describe the main concepts of AST and then overview its applications in the ML4SE domain.

\secpart{Abstract Syntax Tree}

Each programming language has a set of rules---its grammar---that describes the language syntax.
Rules can be viewed as transformations from higher-level language abstractions into sequences of simpler abstractions and code tokens (\eg literals and variable names).
\Cref{fig:rules} shows several examples of grammar rules for method declarations in Java.

The result of parsing source code with the selected grammar is a parse tree. Each intermediate node in a parse tree represents the left-hand side of some rule, and the node's children correspond to the sequence on the right-hand side of the same rule.
Thus, intermediate nodes represent abstractions defined by the grammar and
the leaves in the parse tree correspond to tokens that actually appear in the source code.
\Cref{fig:ast} shows an example of a parse tree built for code fragment shown in \Cref{fig:java_method}.

Parse trees can be quite verbose, so most parsers can further optimize them, \eg by removing unnecessary brackets that are already reflected in the tree structure, or compressing sequences of nodes into new nodes.
After processing the parse tree, the parser constructs an abstract syntax tree (AST) that is usually more compact than the initial tree.

Parsers differ by both the grammar they use and the \linebreak post-processing behaviour.
Post-processing directly depends on the parser's application. For example, PSI~\cite{psi} and JDT~\cite{jdt} are used for language support in IDEs and, therefore, keep all information about the source code including formatting. On the opposite, JavaParser~\cite{danny_van_bruggen_2020_3842713} aims to support complex modifications of Java code, so it optimizes the tree by introducing more layers of abstraction.


\secpart{AST-based Representations in ML Models}\label{sec:ast-for-ml}

A straightforward approach to working with source code in ML models is treating code as a plain text. This approach allows applying models from the NLP domain with close to none modifications in various software engineering tasks, \eg variable misuse, code summarization.
However, as previously discussed, source code has a rich underlying structure that can be represented as an AST. Existing works in the ML4SE domain show that taking code structure into account is indeed beneficial as it leads to significant improvements in multiple SE tasks~\cite{alon2018code2seq, zugner2021codetrans, fernandes2018structured}.

Models that directly support the tree-structured input format, \eg TreeLSTM, can use raw ASTs.
While originally applied to NLP tasks, the TreeLSTM model served as a baseline in multiple ML4SE works~\cite{alon2018code2seq, chen2018tree2tree}. Shido et al~\cite{shido2019automatic} improved the model further by handling an arbitrary number of ordered children via another LSTM cell~\cite{hochreiter1997lstm}.

Another class of models builds their own code representations based on ASTs rather than using the trees as is. Alon et al.~\cite{alon2018general} suggested path-based representation of code.
Path-based representation extracts a set of path contexts from each AST, where each context is a triple of two code tokens in AST leaves and a sequence of intermediate nodes that connect these leaves.
Based on this representation, the authors suggested models for different tasks~\cite{liang2021ast, shi2020pathpair2vec}, including the Code2Vec~\cite{alon2019code2vec} and Code2Seq~\cite{alon2018code2seq} models that show high quality in method name prediction.

While AST represents the syntax of source code, a code fragment can also be represented with a graph structure. Control-flow graph (CFG) contains all possible execution paths of a program. Data-flow graph (DFG) is built from the dependencies between variables in code and their usages.
AST, DFG, and CFG can be combined into a single complex graph, as nodes from CFG and DFG also appear in the code's AST.
Allamanis et al.~\cite{allamanis2017learning} used such graph representation of code to achieve state-of-the-art results in the variable misuse task.
Lately, graph representation was used in the method name prediction~\cite{fernandes2018structured}, type inference~\cite{allamanis2020typilus}, and variable misuse~\cite{Hellendoorn2020Global} tasks to achieve superb results.

AST-based representations of code are not limited to the ones listed above.
Existing works also operate with AST traversals~\cite{Zhang2020retrieval_cs}, apply convolutions over trees~\cite{mou2016tbcnn}, enhance Transformer-based~\cite{vaswani2017transformer} models with information from ASTs~\cite{zugner2021codetrans}. 
Despite the large number of ML4SE works that employ ASTs to improve the results, they rarely motivate the choice of parsers used for AST extraction. Oftentimes, papers either omit the details about the parsing step, or just state the used tool without motivating their choice. In our work, we focus on analyzing the importance of the parser choice in ML4SE and outlining things to consider when making it.

% For example, Zugner et al.~\cite{} in a recent study propose new model architecture, CodeTransformer, that uses relative distances in AST.
% They compare their work with Code2Seq~\cite{}, GREAT~\cite{}, and the model proposed by Fernandes et al.~\cite{}.
% % There is no information about used parsers, but the differences are relatively small: 2-3 points in terms of F1-score for method name prediction.
% % That is make an open question, whether or not changing parser in a data pre-processing pipeline may change the order in model comparison.


==> FSE’22_ Parsers evaluation/sections/03-astminer.tex <==
\section{The \toolname tool}

In order to study the impact of the parser choice on the model's quality, we need a common way to extract input data for models from the source code with different parsers.
To achieve this, we need to run various parsers in a unified manner. In order to ease the maintenance and allow other researchers and practitioners to reuse our data processing pipeline, we integrate all the studied parsers in a single tool, \toolname. 

As a basis for building \toolname, we use PathMiner~\cite{kovalenko2019pathminer} --- a tool for mining ASTs and path-based representations from code in several languages, filtering the data, and storing it in a format suitable for training ML models.
The main advantage of PathMiner is that the tool is designed to be easily extendable. It provides a lot of reusable components for building parsing pipelines, which then can be used for data mining in ML4SE tasks. These components include wrappers for parsers, classes for storing AST vertices, algorithms for filtering, classes for storing the extracted trees.

By using the existing extension points, we create a pipeline that supports parsers directly imported from Kotlin and Java, parsers in other languages that run as separate processes, and grammars for ANTLR and Tree-Sitter. \toolname then runs the parsers to prepare datasets for training and evaluating ML models in the method name prediction task. Using the same pipeline, we run all parsers under equal conditions and ensure reproducibility of our experiments.

\secpart{Multilanguage Parser-agnostic Processing}


Parsers greatly vary depending on their purpose. A parser can be generated from grammar or written from scratch. It can constitute a library, or be a full-fledged runnable tool. The functionality of a parser can range from straightforward construction of parse trees to complex manipulations on source code. Finally, parsers can be written in different programming languages depending on the target applications.
Due to the variability of parsers, supporting multiple parsers in a single data preparation pipeline can be a daunting task. In \toolname, we reuse components of PathMiner and also add new extension points in order to ease the tool's usage for other researchers and practitioners.

In contrast to PathMiner, \toolname supports parsers written in languages that do not run on Java Virtual Machine (JVM). In order to add new languages and parsers, users of PathMiner can either provide a grammar for the ANTLR parser generator or implement an adapter class that wraps a third-party tool written in a JVM-compatible language. However, there are many parsers---both for Java and other languages---that do not provide Java bindings. In order to handle such cases, \toolname has a new entity called \texttt{ForeignParser}. It inherits from the \texttt{Parser} class of PathMiner and can launch standalone tools implemented in other languages to further convert their output into the inner tree structure. A similar idea was used in GumTree\cite{DBLP:conf/kbse/FalleriMBMM14}, a tool that also aggregates multiple parsers and uses them by deserializing their XML output. In our implementation, we use JSON, as this format is more common nowadays.

PathMiner could be easily extended to support new languages by using automatically generated parsers based on ANTLR grammar files. Following this idea, we also add the support of Tree-sitter~\cite{max_brunsfeld_2022_6326492} grammars. Due to the ease of usage, the availability of Python bindings, and the support of many programming languages, Tree-Sitter is commonly being used in ML4SE data mining pipelines. 

Thus, \toolname currently supports:
\begin{enumerate}
    \item parsers that provide JVM bindings;
    \item parsers that can be run as stand-alone processes or wrapped in executable programs with console output;
    \item parsers derived from ANTLR and Tree-sitter grammars.
\end{enumerate}
Importantly, each of these methods has the same API and the work of the parsers is completely hidden from the rest of the \toolname components. For now, our tool already supports 5 different languages with 12 parser/language pairs. While the parser support can be extended, in this study we mainly focus on Java language as we selected it for the evaluation of models.

% In \toolname we keep the file-parsing approach from PathMiner, but we aggregate all tree structure-specific components into a single object --- \texttt{ParsingResultFactory}, which is used for creating \texttt{ParsingResult} --- an abstraction over the parsed file, that able to represent itself in different degrees of granularity (file, method, etc.). In addition, \texttt{ParsingResultFactory} is responsible for data preprocessing before the actual parsing begins, as well as for loading and preparing the parser itself.
% Also, we implemented multi-threaded file processing which significantly speeds up the entire parsing and allows working with large amounts of data.

% This allowed us to draw a clear line between parser-dependent and parser-agnostic components, which in turn facilitated the support and extensibility of the tool.
% \begin{table}[]
% \centering
% \begin{tabular}{c|ccccc}
% \toprule
% {} & \textbf{Java} & \textbf{Python} & \textbf{C/C++} & \textbf{JS} & \textbf{PHP} \\
% \hline
% \textbf{ANTLR}       & + & + &   & + & + \\
% \textbf{GumTree}     & + (JDT, SrcML) & + &   &   &   \\
% \textbf{Fuzzy}       &   &   & + &   &   \\
% \textbf{JavaParser}  & + &   &   &   &   \\
% \textbf{Tree-Sitter} & + &   &   &   &   \\
% \textbf{JavaLang}    & + &   &   &   &  \\
% \textbf{Spoon}       & + &   &   &   & \\
% \bottomrule
% \end{tabular}
% \caption{Supported languages and parsers in \toolname tool.}
% \label{table:parser-support}
% \end{table}

\secpart{Data-processing Pipeline}


\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/pipeline.pdf}
    \caption{
Overview of the data processing pipeline in \toolname. Users can configure the pipeline to suit their needs by providing a YAML configuration file. For example, user can configure the tool to do the following: (1) parse Java code with ANTLR parser, (2) extract ASTs of all methods, (3) remove overriden methods, (4) associate each tree with method name, and (5) store the resulting dataset in JSON Lines format.
}
    \label{fig:astminer-pipeline}
\end{figure*}

% PathMiner is a set of components for creating new tools for converting source code into trees and their derivatives. 
In \toolname, we reuse and improve many components from PathMiner. We combine them into a single pipeline that can be launched from the command line and configured by providing a YAML file.
Novel approaches often rely on large-scale data analysis, thus, we significantly speed up the tool by adding multithreading processing and provide an excessive logging system together with the command-line interface, making it convenient to use \toolname on remote servers.
% and a convenient logging system to track errors and processing progress.
 
% In addition, one of our main tasks was to make the tool convenient not only for use in its current form, but also for extension to new parsers, languages, tasks, and models. Therefore, below we describe the extension points and some parts of our pipeline that can be replaced or extended.

After the parsing stage, \toolname generates a single tree or a set of trees from each file depending on the selected granularity (file or method). The trees have a unified parser-independent form and can then be processed depending on the target task. In order to make \toolname easily extensible to new tasks and ML models, the following processing pipeline consists of several steps which can be configured and changed independently. 
All these steps are represented by simple programming interfaces that could be implemented to extend \toolname with new behaviour. Along with the source code of the tool, we also publish an extensive documentation describing its main components.

\textbf{Label extraction}. Label extractors associate each tree with some string (a label) which can then be used as a target for model training and evaluation. This component of the pipeline can be replaced depending on the task. \toolname currently supports extraction of method names, file names, and parent folder names.

\textbf{Filtering}. At the next stage, \toolname applies filters to all the extracted trees and labels. Label filters can be used to remove samples with the desired labels that cannot be supported by a model, \eg names in unsupported languages, too long or too short names. Tree-level filters can be either structural or content-based. Structural filters remove samples based on the AST characteristics: depth, number of vertices. Content-based filters operate with the tree itself and filter samples by annotations (\eg removing overridden methods or tests), modifiers (\eg removing abstract methods), and the size of the method's body.

In order to avoid implementing a separate set of filters for each parser, we accompany parsed trees with a set of features pre-computed at the parsing stage. This set includes both external and internal features. External features include names of the file and enclosing elements (\eg classes and enumerations). Internal features are function parameters, its name, modifiers, annotations, and others. These features are stored in a parser-independent form, which allows users to implement new filters without manual analysis of the parsed structure. % forget about a specific data structure during filtering. % Thus, if the developer has enough current features, then he may not think about the specific structure of the trees. If filtering for a specific task with the current features is not possible, then it will be enough to implement only those that are necessary for the developer. What's more, these features can then be reused in other filters, which is why we strongly support this, and any other parser-dependent contributions to our tool.

\textbf{Storing}. At the last stage of the pipeline, we convert the trees to the selected format and finally save the dataset on disk. For storing the data, we mostly reuse components of PathMiner, but also add the ability to compress trees before storing. In addition, we save metadata alongside with the mined dataset, such as the origin of the tree (\ie path to the enclosing file) or the location of the corresponding code snippet in the file.

To compress trees, we use the algorithm presented by Yin et al.~\cite{yin2017syntactic}. The authors use production rule closures and concatenate the names of the rules into a single vertex type. In order to make the process parser-independent, we imitate this algorithm by compressing ``bamboos'', \ie sequences of nodes in a tree that have a single child each, into single nodes in the already generated AST.

% Along with the stored dataset, we save metadata in JSON Lines format, where each line corresponds to one extracted sample. Metadata helps to further track all the trees. For example, it can be used to collect detailed statistics on which samples are the hardest or the easiest for the models.

==> FSE’22_ Parsers evaluation/sections/04-experiments.tex <==
\section{Experimental setup}\label{sec:motivation}

\secpart{Research Questions}
% The use of a specific tree structure for a specific model and task has not been fully studied. In this work, by comparing the set of parsers on machine learning models, we tried to study whether the choice of tree structure is essential for learning. More specifically, we ask the following research questions:
With this study, we aim to investigate the importance of the initial source code parsing step for the machine learning on source code algorithms.
Moreover, we focus on the differences of how source code is parsed and how these differences affect the final performance of ML models.
We formulate the following research questions:

\begin{itemize}
    \item \textbf{RQ1:} Is there any statistical difference in the ASTs produced by different parsers?
    \item \textbf{RQ2:} How does the parser selection affect machine learning models that take into account tree structure of code?
    \item \textbf{RQ3:} Alongside with the model quality, what else researchers and practitioners should take into account when choosing a parser for their data-processing pipeline?
\end{itemize}

% Almost always, researchers use third-party parsing tools to obtain AST. The answer to RQ1 will let us know if this results in different tree structures being used in different studies.
With RQ1, our goal is to understand whether different parsers indeed lead to varying characteristics of model input.

% Since the parser only affects how the program is represented as a tree, the answer to RQ2 will let us know if the structure of the tree affects learning.

% A positive response to RQ2 in combination with a positive response to RQ1 would mean that the results of the study depend on the structure of the trees used in training. A positive answer to RQ1 and a negative answer to RQ2 will indicate the possible independence of the learning quality from the structure of the tree. A negative response to RQ1 for any response to RQ2 will indicate the need to select other tools or languages as targets for comparison.
By answering RQ2, we aim to understand whether the differences in trees produced by different parsers lead to changes in the quality of machine learning models.
If the answer is positive, further research should pay attention to the choice of a parser in order to maximize the performance of the studied models and to ensure fair comparison.

% RQ3 is practical. Answering it, we want to tell the researchers which of the reviewed parsers is better to take, depending on the use case.
% RQ3 studies the correlation of AST characteristics from RQ1 and ML models quality from RQ2.
% By investigating this, we aim to find crucial features that should be considered while choosing a parser for the data-processing pipeline. 
In RQ3, we address practical features of code parsers, such as their speed, size of the generated datasets, and language support. These aspects become important when choosing between parsers that allow models to achieve similar quality.

% \secpart{Language}
% Java is a popular language (common target for analysis)
% Very old and complex (many tools)
% common target for research


% and articles with the results of which we can compare our own.

\secpart{Parsers}
As a target programming language for this study, we use Java due to its common adoption in the ML4SE domain. Java is a fairly common target for syntactic and semantic analysis, as well as for research works on code summarization~\cite{alon2018code2seq, fernandes2018structured}, code generation~\cite{wei2019cg-cs}, and others~\cite{liang2021ast}.
Also, due to the language's popularity, long history of development, and numerous applications, there exist a lot of different parsers for Java.

There are many tools that convert source code into a tree structure. The main examples are interpreters and compilers that use it to make the code executable. Other examples are refactoring and code highlighting systems (\eg PSI trees in the IntelliJ Platform), algorithms for comparing source code~\cite{DBLP:conf/kbse/FalleriMBMM14}, algorithms for finding duplicates in code~\cite{tairas2006phoenix}, and other tasks where program structure is important. Due to the variety of applications, there are many parsers for different scenarios.
For this work, we selected the following parsing tools and libraries:
    
\textbf{ANTLR}~\cite{10.5555/2501720} --- a parser generator that takes a grammar for the target language as input and generates a parser implementation in one of the supported languages. In this work, we use ANTLR with an open-source grammar for Java.\footnote{Java 8 ANTLR grammar: \url{https://github.com/antlr/grammars-v4/tree/master/java/java8}}

\textbf{Eclipse Java Development tools (JDT)}~\cite{jdt} --- a set of plugins for Eclipse IDE that are responsible for supporting Java. Based on JDT, the IDE can highlight Java code, refactor it, perform different checks, and more.
We use GumTree~\cite{DBLP:conf/kbse/FalleriMBMM14} Java API to add JDT support to \toolname.   

\textbf{JavaLang}~\cite{tunes} --- an open-source library written in pure Python for working with the Java 8 source code. Due to the implementation in Python, JavaLang can be easily integrated into ML and data science pipelines. The library focuses on parsing and does not provide tools for further manipulations with the extracted trees.

\textbf{JavaParser}~\cite{danny_van_bruggen_2020_3842713} --- a Java library for parsing, transformation, and generation of Java code. It allows analyzing Java programs, generating boiler-plate code, and focuses on complex manipulations with the generated ASTs. Notably, it has been used in some of the previous ML4SE studies~\cite{alon2018code2seq, zugner2021codetrans,fernandes2018structured}.

\textbf{Program Structure Interface (PSI)}~\cite{psi} --- similar to JDT, it is a tool that is responsible for the language support in IDEs built upon the IntelliJ Platform. It allows manipulation of source code inside the IDEs and their plugins, running inspections, refactorings, and more.
We use PSIMiner~\cite{psiminer} to extract PSI trees from code.

\textbf{Spoon}~\cite{pawlak:hal-01169705} --- an open-source library for parsing, rewriting, transforming, and transpiling Java code. In contrast to previous tools, it was developed in the research community and since then has been used in numerous works on refactoring and program repair~\cite{xuan2016nopol, martinez2016astor, long2017automatic}.
% It is one of the most interesting candidates, since it has practically no information about it's use in the ML problems.

\textbf{SrcML}~\cite{collard2013srcml} --- a lightweight tool for analyzing and manipulating source code. It allows transforming C, C++, and Java code by using trees in a native SrcML format inspired by XML. The authors provide a set of tools for further manipulation of the extracted trees: static type resolution, pointer analysis, builder of UML diagrams, etc.
To support this parser in \toolname, we also use GumTree.

\textbf{Tree-Sitter}~\cite{max_brunsfeld_2022_6326492} --- a parser generator focused on the usage in text editors and IDEs in order to provide features like syntax highlighting in real time. Due to the need for real-time usage, Tree-sitter can parse code incrementally, is fast and robust when parsing unfinished code. Similar to ANTLR, we use its most popular grammar for Java 8.\footnote{Java 8 Tree-sitter grammar: \url{https://github.com/tree-sitter/tree-sitter-java}}

\smallskip

The chosen parsers target different applications. Each parser has its own features: from being lightweight and fast, to supporting complex manipulations of ASTs. This diversity allows us to assess whether ASTs extracted with different parsers are similar or they can affect the quality of ML models working with source code.

\secpart{Models}
% It should be noted that machine learning models do not have a uniform approach to working with AST. Models can transform trees, collect additional information, or completely convert trees to a new format. Therefore, to get the answer to RQ2, we used two different approaches and conducted 5 training iterations using each of the 8 parsers. We ended up with 80 different models to analyze.

In this work, we compare two different ML models, TreeLSTM~\cite{DBLP:journals/corr/TaiSM15} and Code2Seq~\cite{alon2018code2seq}, that can solve software engineering problems by working with tree-based representation of code or its extensions.
With this, we aim to make a diverse selection from the point of model architecture and tree input format.

\textbf{TreeLSTM.} Originally created for natural language processing, the TreeLSTM model was then reused and adapted for working with source code~\cite{alon2018code2seq}.
Although this model is simpler and shows inferior quality compared to the novel approaches, TreeLSTM works directly with tree representation of code.
This is crucial for our research, since it allows comparing the impact of parsing differences directly, without additional transformations of trees (\ie adding new edges in DFG or CFG~\cite{allamanis2017learning}).

% Since then, it has ceased to be used alone and instead is now very often used to generate embeds or sequences for other more complex models.

% The main feature for our study is that the input for this model is trees, which do not require additional transformations. Thus, the model will directly depend on the structure of the trees.

\textbf{Code2Seq.} On the other side, Code2Seq is a popular model showing good results in many SE applications~\cite{alon2018code2seq, nagar2021code, Zhang2020CBPath2Vec}.
This model receives information about source code from a path-based representation, \ie a set of contexts where each context is a triple of tokens in two leaves in a tree and a sequence of intermediate nodes on a path between them. As Code2Seq does not work directly with ASTs, we can assess whether the choice of a parser can affect the models that use code representations derived from the ASTs.

% the authors compose a bag of paths between nonterminals, and then model trains on each function, choosing $k$ random paths from the bag. This approach gets better results in method name prediction problem, meanwhile on of it's biggest assets -- learning on paths -- can be influenced by parsing instrument.

% For this study we use our own implementation of the model. For each function we took up to 1000 paths, each path having maximum length of 9 and width of 2.

\secpart{Dataset}\label{sec:dataset}

In order to ensure correctness of the results and reduce randomness, we run each model five times with different random seeds for each parser. Thus, train and evaluate models $80$ times in total (2 models $\times$ 5 random seeds $\times$ 8 parsers). Due to the high number of experiments, initially we decided to use the \emph{Java-small} dataset~\cite{allamanis2015acc_method_names}. In our case, using larger datasets such as \emph{Java-med} and \emph{Java-large} is too computationally intensive as they are 5 to 30 times larger than \emph{Java-small}.

However, our experiments and previous experience with \emph{Java-small} suggest that evaluating the models on this dataset comes with two important limitations:
\begin{enumerate}
    \item The models' quality reported on the validation data weakly correlates with the results on the testing data and is often way lower.
    It makes tuning of hyper-parameters based on the validation quality unreliable.
    % It makes early stopping based on validation unreliable.
    \item Model evaluation on \emph{Java-small} is not robust, with small model modifications leading to large deviations in the final metrics. As a result, evaluation on this dataset often disagrees with larger datasets in terms of relative model ranking.
\end{enumerate}

Our investigation of these issues suggests that a significant disadvantage of \emph{Java-small} is that both its validation and testing parts consist of a single project each.
Judging models quality by evaluating on a single project might lead to non-representative results since every project is unique in some way.
Moreover, the \texttt{libgdx} project that constitutes the validation set is not a typical Java project, with more than 45\% of code written in C and C++, which might explain the discrepancy between the validation and testing results. 

In order to deal with this issue, we compile a new dataset called \javanorm that has a size comparable to \emph{Java-small}, but aims to mitigate its issues. \javanorm contains five projects in both validation and testing parts (see \Cref{table:data_intersected} for the list of projects). The training part of the new dataset includes ten open-source Java projects. As the set of projects in both testing and validation is more diverse, evaluation on \javanorm is more representative and robust.

We collect projects that are publicly available on GitHub.\footnote{GitHub: \url{https://github.com/}} 
While collecting the data, we respect all intellectual rights and select only the projects whose licenses allow to reuse the code for further analysis.
We collect projects that have one of the following licenses: Apache-2.0, MIT, or BSD-3.0.
We consider projects that are not forks and have at least 20MB of Java code.
Across all projects that meet these criteria, we take the ones with the highest numbers of GitHub stars.

We make \javanorm publicly available via Zenodo.\footnote{\javanorm: \url{https://doi.org/10.5281/zenodo.6366599}} As it mitigates some issues of \emph{Java-small} while being comparable in size, we believe that the dataset can be useful for future research in the method name prediction and other ML4SE tasks.

\secpart{Evaluation Scheme}
% method name prediction problem
% good benchmark for how model summarizes code
% used a lot, so the results can be applied to many existing studies

In the rest of this section, we describe the evaluation scheme we use to evaluate the impact of parsers on models' quality and answer the research questions.

\textbf{Tree comparison.}
In order to verify whether trees built by different parsers are similar or not, we compare them by several metrics: tree depth, size, branching factor, etc. The values of a certain metric for different trees produced by the same parser can be viewed as a distribution of an unknown form.
Therefore, to compare trees produced by different parsers, we can compare the distributions of their metrics.
%differences in the trees from different parsers comes down to the compare the distributions of tree-based metrics.

There exist multiple approaches to compare numerical distributions.
One of the most popular is the Student's t-test~\cite{student1908probable} that tests the hypothesis of mean equality between Normal distributions.
Although values of a certain metric for a single parser are not normally distributed, with a dataset of 300 thousand trees, we can apply the Central Limit Theorem and work with this test.

\textbf{Method name prediction.}
As a benchmark for our study, we select the method name prediction problem.
% More formally, it sounds like: using the method name, parameters, annotations, modifiers, and return type (in whatever form), the model must generate the name that best suits the given method.
More formally, the model should generate a name of the method given its body and signature with the original name being replaced with a stub token.
This task is a common benchmark for analyzing model capabilities in code understanding and summarization~\cite{alon2018code2seq, fernandes2018structured, zugner2021codetrans}.

% Moreover, since it is often used in model evaluation, the result of this article can be applied to several existing studies at once.

As a de-facto standard, we treat the method name prediction task as a sequence generation problem.
In this setting, each method name is split into a sequence of sub-tokens by CamelCase or snake\_case.
Models then generate sub-tokens one by one, taking the code snippet and already predicted sub-tokens into account.

\textbf{Intersection of datasets.}\label{sec:dataset-intr}
As different parsers use different underlying algorithms, they might parse different sets of files or methods from the same code corpus. It might happen due to several reasons: some parsers fail for specific files due to the presence of unexpected symbols, syntactically incorrect or incomplete code, unsupported versions of Java, etc. Also, processing of trees for each parser requires significant manual parser-specific work (\eg to correctly split the trees into methods or extract modifiers) which might fail in corner cases. As a result, the set of parsed ASTs from the same initial code dataset slightly differs from parser to parser.
% Therefore, extracting ASTs from the same source code corpus but with different parsers may lead to a slightly different number of examples in finite datasets.

In order to correctly answer our research questions, the resulting datasets for all the parsers must contain trees for exactly the same set of methods. Otherwise, the diversity in the models' quality may be attributed to the differences in the training and testing sets.
In order to mitigate this, we \textit{intersect datasets}, \ie  we keep only those methods that may be successfully parsed by each parser. For this, we store a source range for each extracted method --- the exact position where this method appears in the source code. Based on the source ranges, we match methods extracted by different parsers. In total, we dropped less than 1\% of the methods after the intersection, \Cref{table:data_intersected} provides information about the final dataset.

\begin{table}[htbp]
    \centering
 \begin{tabular}{c|ccc}
 \toprule
                           & \textbf{Training}   & \textbf{Validation}     & \textbf{Testing}             \\ \hline

\multirow{10}{*}{\textbf{Projects}} & cassandra        & \multirow{2}{*}{buck}   & \multirow{2}{*}{bazel}    \\
                           & gocd             &                         &                           \\
                           & gradle           & \multirow{2}{*}{dl4j}   & \multirow{2}{*}{dbeaver}  \\
                           & hbase            &                         &                           \\
                           & kafka            & \multirow{2}{*}{druid}  & \multirow{2}{*}{guava}    \\
                           & pentaho-kettle   &                         &                           \\
                           & presto           & \multirow{2}{*}{flink}  & \multirow{2}{*}{keycloak} \\
                           & pulsar           &                         &                           \\
                           & spring-framework & \multirow{2}{*}{j2objc} & \multirow{2}{*}{quarkus}  \\
                           & tomcat           &                         & \\ \hline
\begin{tabular}[c]{@{}c@{}}\textbf{Number of}\\ \textbf{methods}\end{tabular}                & 295,425          & 187,717 & 144,656                  \\ 
\bottomrule
\end{tabular}
    \caption{Sets of projects and number of methods (after the intersection step) in training, validation, and testing parts of \javanorm.}
    \label{table:data_intersected}
\end{table}

\textbf{Metrics.}
The most popular approach to measure quality of method name prediction is F1-score~\cite{allamanis2015acc_method_names}.
Originally applied for classification, it was adopted to evaluate the quality of generated sequences. F1-score is a harmonic mean of precision and recall.
Given two sequences, ground truth and prediction, precision is a proportion of sub-tokens from the predicted sequence that appear in the ground truth.
Recall, as an opposite, is a proportion of correct sub-tokens that appeared in the predicted sequence.
Finally, F1-score is a harmonic mean of these two values.

Although F1-score is a popular metric, it also has disadvantages, \eg it does not take into account the order of sub-tokens. While for some method names (\eg \texttt{arraySort} and \texttt{sortArray}) it does not affect the meaning, in other cases it might alter it (\eg \linebreak \texttt{implementationParser} and \texttt{parserImplementation}).
% To cover this gap, different metrics from NLP may be applied.
Recently, Roy et al.~\cite{roy2021reassessing} evaluated the applicability of multiple metrics from the NLP domain in code summarization tasks. Specifically, the authors evaluated METEOR~\cite{banerjee2005meteor}, BLEU~\cite{papineni2002bleu}, Rouge~\cite{lin2004looking}, ChrF~\cite{popovic2015chrf}, and BERTScore~\cite{zhang2019bertscore}.
Judging by their results, ChrF~\cite{popovic2015chrf} appears to be the most robust metric for code summarization, so we employ it in our study alongside the F1-score.

\textbf{Model comparison.}
The answer to RQ2 requires pairwise comparisons of independent models trained and tested on the same set of methods, but with data prepared by different parsers.
To do so, we run the paired bootstrap test~\cite{Efron93bootstrap} over the predictions of two models.
The test resamples the result pairs with replacement multiple times and compares average results of the models on the sampled examples.
The probability of one model beating the other is a ratio of how often the average score for this model is better than for the other to the total number of runs.


==> FSE’22_ Parsers evaluation/sections/05-results.tex <==
\section{Results}\label{sec:results}

We use the described evaluation scheme for per-parser analysis of the produced ASTs and further comparison of two ML4SE models: TreeLSTM~\cite{DBLP:journals/corr/TaiSM15} and Code2Seq~\cite{alon2018code2seq} on the method name prediction problem. We use a newly collected \javanorm dataset, leaving only the methods successfully processed by all the studied parsers.


\textbf{RQ1: Is there any statistical difference in the ASTs produced by different parsers?}\label{sec:tree_analysis}

\begin{table*}[]
    \centering
    \input{tables/parser-diff}
    \caption{
On the left-hand side: median values of the computed metrics for each parser. TS -- tree size, TD -- tree depth, BF -- branching factor, UTP -- unique types, UTK -- unique tokens.
On the right-hand side: parsers' features that can be considered when building a data processing pipeline.
\\
$^*$We extract PSI trees with PSIMiner~\cite{psiminer} rather than with \toolname. PSIMiner is slower compared to \toolname as it opens each project in IntelliJ IDEA, which introduces a significant time overhead.
    }
    \label{table:tree-stats}
\end{table*}

\begin{table*}[]
    \centering
    \input{tables/ttest}
    \caption{Tree metrics that are similar for trees produced by each pair of parsers according to the Student's t-test with $p$-value 0.01. For example, trees built by ANTLR and Spoon are similar w.r.t. tree depth. %TS -- tree size, TD -- tree depth, BF -- branching factor, UTP -- unique types, UTK -- unique tokens.
    }
    \label{table:ttest}
\end{table*}


In order to answer the first research question, for each tree, we compute the following set of metrics:
\begin{itemize}
    \item \textbf{tree size} (TS) --- number of nodes in a tree;
    \item \textbf{tree depth} (TD) --- number of nodes in a path from the root of a tree to its deepest node;
    \item \textbf{branching factor} (BF) --- mean number of children in non-leaf vertices of a tree;
    \item \textbf{unique types} (UTP) --- number of unique types of intermediate nodes used in an AST, lower values correspond to a higher level of abstraction used in a parser as it can represent the same code fragment in a more compact way;
    \item \textbf{unique tokens} (UTK) --- number of unique sub-tokens in AST leaves, lower values also reflect higher level of abstraction (\eg whether parser keeps binary operators as tokens or as node types).%, lower values correspond to a higher level of abstraction.
\end{itemize}

The first three metrics aim to reflect the tree structure and estimate how different the trees are size-wise.
The latter two metrics analyze the content and abstraction level of trees produced by different parsers.
\Cref{table:tree-stats} provides quantitative information about the computed metrics for each parser.

After computing the selected five metrics for trees built by each parser, we apply the Student's t-test~\cite{student1908probable} to determine whether the distributions differ for each pair of parsers.
We consider distributions to be significantly different if the corresponding \textsc{p-value} is less than $0.01$, \ie we consider distributions different only if the probability of a mistake is less than 1\%.
% Full tables with pairwise comparisons between each two parsers for all metrics take a lot of space and mostly contain close to zero values.
According to the conducted statistical tests, all parser pairs produce trees different by at least three metrics. \Cref{table:ttest} shows with respect to which metrics the output of two parsers is similar for each pair of parsers.

\begin{tcolorbox}[enhanced jigsaw,colback=bg,boxrule=0pt,arc=0pt]
\textbf{Take away 1.} By applying different parsers to the same code fragment we get different trees both in terms of structure (\ie tree size, depth, and branching) and in terms of content (\ie the number of unique types and tokens in the trees). Although some parsers produce trees that are similar by one or two metrics, for all parser pairs trees differ significantly in various ways.
\end{tcolorbox}


\textbf{RQ2: How does the parser selection affect machine learning models that take into account tree structure of code?}

Since RQ1 shows that different parsers produce trees with different characteristics, it is necessary to study whether it affects the quality of models that utilize these trees. 
For that, we train both models, TreeLSTM and Code2Seq, on the datasets produced by each parser.
To get reliable results, we train each model-parser pair five times with different random seeds.
Therefore, we train and evaluate $80$ models overall. \Cref{table:model-results} shows mean values and variance of metrics for each model-parser pair.

\begin{table*}[]
    \centering
    \input{tables/model-results}
    \caption{Quality of method name prediction for TreeLSTM and Code2Seq models on the data extracted with the studied parsers.}
    \label{table:model-results}
    \vspace{-0.2cm}
\end{table*}

\newdimen\figrasterwd
\figrasterwd\textwidth
% \vspace{-0.5cm}
\begin{figure*}[ht]
    \centering
    \parbox{\figrasterwd}{
        \centering
        \subcaptionbox{
Paired bootstrap for TreeLSTM model.\label{fig:bootstrap-treelstm}
}
        {\includegraphics[width=0.77\textwidth]{figures/bootstrap-treelstm.pdf}}
        \subcaptionbox{
Paired bootstrap for Code2Seq model.\label{fig:bootstrap-code2seq}
        }
        {\includegraphics[width=0.77\textwidth]{figures/bootstrap-code2seq.pdf}}
    }
\caption{
Results of pairwise bootstrap tests for TreeLSTM and Code2Seq models. The numbers are probabilities of one model beating another with random initialization and on a random subset of data. Colors are added for clarity.\label{fig:bootstrap}
}
% \vspace{-0.5cm}
\end{figure*}

The direct comparison already shows the difference between parsers for both models.
An accurate parser choice can increase F1-score by up to $27\%$ for TreeLSTM and $5.5\%$ for Code2Seq compared to the worst performing parser. For ChrF the results are similar, with $31\%$ and $8\%$ increase for TreeLSTM and Code2Seq, respectively.
While the absolute differences might seem low, we argue that they cannot be ignored in current ML4SE research. Nowadays, most works compare the models by directly comparing metric values averaged over the testing dataset (average F1-score in the case of method name prediction). For example, in the recent works on method name prediction~\cite{zugner2021codetrans,fernandes2018structured}, the differences of less than 2 percentage points in F1-score between different models and different model variations are considered significant, while some of the compared models heavily rely on code structure. Thus, the observed differences in metrics depending on the parser are comparable to the values considered significant in modern works.

In order to further ensure correctness of the results, we also conduct paired bootstrap tests for the trained models with respect to F1-score.
For each pair of parsers and random seeds, we run their pairwise comparison with 1,000 bootstrap resamples, 25,000 resamples in total (5 random seeds for both parsers). We then estimate the probability of one parser beating another as the percentage of resamples where it has a higher average score.
\Cref{fig:bootstrap-treelstm} and \Cref{fig:bootstrap-code2seq} provide the computed probabilities for both models and all analyzed parsers. Given the current approach to model comparison (\ie direct comparison of averaged metrics over the testing dataset), the values can be interpreted as the probability of the same model with one parser showing better quality than with another one.

% We consider two models the same in terms of quality if the probability of one beat another in the range between $0.35$ and $0.65$ that is indeed uniformly splits possible probabilities into three sets: lose, draw, and win.
% Other probabilities means that one model definitely beat or lose to another, and the results can not be interpreted as the same.


Firstly, the bootstrap results suggest that parsers indeed have an impact on the model quality. Otherwise, all the pairwise winning probabilities would be close to 50\%. Secondly, for both models, there exists a parser (JavaParser for TreeLSTM, JDT for Code2Seq) that beats the others most of the time and can be treated as a superior choice when working with this model. Also, there are parsers for each model (\eg ANTLR, JavaLang, and JDT in the case of TreeLSTM) that show similar performance to each other and can be used interchangeably depending on the existing limitations (\eg speed, ease of integration into the mining pipeline). Finally, for the two studied models, the relative ordering of parsers differs. While for TreeLSTM JavaParser is the best choice, and Spoon and PSI show poor quality, for Code2Seq it is JDT which is the best, and Spoon and Tree-sitter are falling behind the others. 
% At first, there are some parsers that didn't show any superiority to other parsers, \eg Spoon and PSI.
% On the other hand, there are small clusters that show close results to each other and different from other parsers, \ie ANTLR-JavaLang-JDT for TreeLSTM model and JavaParser-SrcML-ANTLR for Code2Seq.
% Finally, there is no parser that always shows the best quality, therefore, there is no ``silver bullet'' for choosing the correct way of preprocessing data.

Combining the changes in models' quality with the tree metrics computed in RQ1 allows us to make assumptions about the nature of the changes.
We notice that shallower trees generally lead to better model performance, which is intuitive since ML models may struggle to pass information on long distances.
Another observaion is that the small size of the trees combined with a higher level of their abstraction (fewer unique types and tokens) helps JavaParser, JavaLang, and JDT consistently outperform the others.

\begin{tcolorbox}[enhanced jigsaw,colback=bg,boxrule=0pt,arc=0pt]
\textbf{Take away 2.} The choice of a parser for data preprocessing impacts the model's quality.
Although some parsers show dominance over others, the optimal choice is specific to each model.
Without additional information about the model, parsers that produce compact trees with higher level of abstraction are more preferable. %However, when making the choice, researchers should pay attention to the nuances of the specific model at hand.
% In order to correctly assess models, researchers should pay attention to the parser choice and select the most suitable one (\eg producing shallower or larger trees) depending on the nuances of the specific model or experiment with different parsers. 
% All in all, switching between parsers may increase or decrease quality and should be considered while developing a preprocessing pipeline.
\end{tcolorbox}

\textbf{RQ3: Alongside with the model quality, what else \linebreak researchers and practitioners should take into account when choosing a parser for their data-processing pipelines?}

% Statistical descriptions of trees and final model qualities show that more vertices in a tree lead to poorer model performance.

% In RQ2 we determined that parser choice affects model quality. However, aside from raw performance, there

For both models, there exist groups of parsers showing similar performance. When choosing between such parsers, aspects other than raw model quality should be taken into consideration.
%(\eg speed of data processing). Aside from the raw model quality, there are other aspects that researchers should take into account when choosing an appropriate parser. 
Depending on the task at hand, the size of the dataset, and target programming languages, different parsers might become more or less suitable. 

When dealing with large-scale datasets, the parser's speed might become a bottleneck. \Cref{table:tree-stats} shows the average number of processed examples per second for all the parsers.
To measure this, we run \toolname multiple times for each parser with a task of preparing data for the TreeLSTM model, for which parsing is the most time-consuming stage of the pipeline.
The fastest parsers considered in this study---JDT and JavaParser---are more than 8 times faster than JavaLang and more than 6 times faster than Tree-sitter.

Another resource-related issue is the memory required to store the resulting dataset. It might affect the speed of model training: smaller datasets are faster to read from drive, and in some cases can be loaded directly into RAM. Memory consumption directly depends on the size of the produced trees. The Spoon and PSI parsers generate 2 to 4 times larger trees compared to others. The TS column in \Cref{table:tree-stats} provides average tree sizes for different parsers, which allows to approximate the size of the processed dataset.
% During direct inference of the model, it is necessary to quickly obtain code snippet AST and give programmer appropriate hints. While doing our research, we noticed that \textbf{JavaParser} is the \textbf{fastest} in terms of the number of processed files per second, and \textbf{JavaLang} and \textbf{PSI} are the slowest.

Support of multiple programming languages allows the whole learning pipeline to be less dependent on a specific language and thus be more extensible. Moreover, it is necessary for training multi-language models~\cite{feng2020codebert}. Parser generators like ANTLR\footnote{ANTLR supported languages: \url{https://github.com/antlr/grammars-v4}} and Tree-Sitter\footnote{Tree-Sitter supported languages: \url{https://tree-sitter.github.io/tree-sitter/\#available-parsers}} can support any language if the appropriate grammar is available, making them the most flexible choice. In addition to Java, SrcML also supports C, C++, and C\#.
While, PSI works for all the languages supported by IntelliJ-based IDEs and their plug-ins, extraction of PSI for each language requires manual work to extend PSIMiner. Currently, PSIMiner supports Java and Kotlin.
The rest of the tools that we consider support only the Java language.

Finally, since most ML pipelines use Python as the main language, Python bindings might be convenient to interact with the parser directly. Out of the considered parsers, only ANTLR, Tree-Sitter, and JavaLang provide the necessary bindings, while the other can only be used with JVM.

\begin{tcolorbox}[enhanced jigsaw,colback=bg,boxrule=0pt,arc=0pt]
\textbf{Take away 3.} In addition to the parser's impact on the model quality, there are other aspects that researchers and practitioners might consider while selecting a parser: speed, language support, ease of usage.
The exact limitations on the parser choice come from the studied problem, usage scenarios, and the selected model architecture. In order to choose a parser for data processing, researchers should first identify parsers that are applicable in their situation, and then treat the applicable parsers as a hyperparameter. The final choice can be made via empirical validation or by carefully studying features of trees produced by each parser and the nuances of a particular ML model. 
%  researchers should clearly communicate the reasons for parser choice.
\end{tcolorbox}

% For example, developing multi-language models requires a parser that can work with all necessary programming languages.
% To provide information about selecting the parser with respect to practice use-cases, we aggregate most valuable information into ~\Cref{table:practice-perfomance}.

% \begin{table*}[]
%     \centering
%     \input{tables/perfomance}
%     \caption{Parsers comparison by practical use-cases}
%     \label{table:practice-perfomance}
% \end{table*}


==> FSE’22_ Parsers evaluation/sections/06-discussions.tex <==
\section{Discussion and Future Work}\label{sec:discussions}

The conducted analysis of the impact parsers have on ML4SE models shows that it can lead to significant deviations in the models' performance. For TreeLSTM, a model that directly works with ASTs, the difference in F1-score can be as large as 27\% depending on the parser. For Code2Seq, a model that uses path-based representations derived from ASTs, the effect is smaller, but it is still comparable to the metric differences considered to be significant in recent works.

% Benchmarking on a method name prediction problem shows that differences between one model with different parsers may reach enough values to change the order of latest models (the case from \cref{sec:ast-for-ml}).
Judging by the results, researchers and practitioners should pay closer attention to parser selection when designing their data processing pipelines. Although some use cases imply strict limitations on the used parser, in most cases there exist several parsers to choose from. In such cases, the choice of a parser should be interpreted as one of hyperparameters when training a model, thus it requires either clear reasoning or empirical validation.

In this work, we focused on the method name prediction task and the Java language. However, the usage of structured code representations proved to be helpful in other tasks as well: variable misuse prediction~\cite{Hellendoorn2020Global}, clone detection~\cite{liang2021ast}, comment generation~\cite{li2020deepcommenter}, etc.
Also, Java is not the only language that has a variety of parsers --- it is also the case for C/C++, Python, PHP, and others. Extension of this study to other tasks and languages is an important topic for future work.

Most structured representations of source code utilize ASTs in some way, but they are not limited to it. Researchers also used data-flow graphs, control-flow graphs, program dependence graphs, and even combined all of them into a single complex structure~\cite{allamanis2017learning, allamanis2020typilus}. As it is the case with parsing, the process of building other structural representations is also non-straightforward. Possible differences in this process range from the exact set of dependencies included in the graph to the specific tools used to extract them. We leave careful analysis of the data preparation process for more complex code representations and its impact on model quality for the future work.

% Aside from the impact on models' quality, parsers have other distinctive features: language support, supported bindings, speed. In our work, we outlined several comparison points for parsers in case when they lead to similar model performance.


% In this section, we answer some of the questions that we had after receiving the results. Some of them arise from a lack of attention to this area, which leads to the need to continue this research.

% \secpart{Q1. Do the same results apply to other models and languages?}

% As we said earlier, in general it's impossible to find the perfect parser. Different tools will be suitable for different tasks. However, it is not a fact that the choice of a parser is important for all models. The same can be said about the programming language.

% We do not exclude the possibility that there are languages and models that the parser will not have a significant impact on.

% It is also possible that the perfect tool can be found for some languages. This can happen if the language is not very popular and there are few parsing tools for it.

% Thus, the next step for this study will be expansion to new models and languages, which is possible due to the competent integration of all used components in \toolname.

% \secpart{Q2. Do the results depend on how the parsers are used?}

% By converting the trees to the internal \toolname structure, we tried our best to get the most informative trees. However, we do not exclude that we could have missed some information that affects learning. It is possible that by doing the analysis much more thoroughly, we can improve the results we have obtained.

% It is also possible to reduce the percentage of files that are not supported by the parser by using a different version of the components or different launch configurations.

% Because of this, all the code for integrating parsers is completely open source. Thus, the authors of these parsers will be able to make comments and suggestions on how to work with their tools.

% \secpart{Q3. What happens if you train the model on other data?}

% In this study, we trained all models on a relatively small dataset. It is possible that on larger data the difference can both decrease and increase.

% A decrease will indicate that the difference in the structure of trees affects only the initial stages of training, and when the model reaches a certain limit, it will be able to completely obtain all the information from the trees. It should be noted that choosing the optimal parser still makes sense. By choosing the best parsing tool, you can achieve convergence much faster.

% On the other hand, if different tree representations really affect learning not only at the initial stage, but throughout the entire training, then the choice of the optimal parser becomes an important hyperparameter for discussion.

% Also, in addition to the size of the dataset, the data filtering parameters, the division of projects into holdouts and the choice of the projects themselves for training can vary. All this in theory can affect our results and is the goal of our further research.

% \secpart{Q4. Do you need to select hyperparameters for a specific parser?}

% We trained all models on the same set of hyperparameters that keep data loss to a minimum for each parser. However, in theory it is possible to select hyperparameters for each parser and thus obtain different results.

% Like all previous questions, this can be answered by conducting more experimentation, which indicates the need for more extensive research in this area.

==> FSE’22_ Parsers evaluation/sections/07-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

With this work, we present an analysis of how the selection of a parsing tool for AST extraction can affect the quality of Machine Learning models that rely on structured representations of code.
We demonstrate that the usage of different parsers leads to the differences in AST characteristics, both in terms of structure (\ie tree size or depth) and content (\ie number of different node types or tokens).
These differences further impact the quality of ML models.
For the TreeLSTM model that works directly with the trees, the difference can reach up to $27\%$ of F1-score and $31\%$ of ChrF for the method name prediction task.
For Code2Seq, a model that uses path-based representation derived from the AST, the difference is less drastic, only about $5\%$ of F1-score and $8\%$ of ChrF, but it is still significant.

In order to simplify experiments with different parsers, we develop \toolname, a tool that can run various parsers in the same manner. In order to run experiments with different parsers, users have to change a single value in the YAML configuration file. The tool facilitates the end-to-end creation of machine learning datasets from source code.
\toolname already supports 5 different languages with 12 parser-language pairs and can be extended to new parsers and languages.
Our tool is publicly available at \url{https://doi.org/10.5281/zenodo.6366591}.
% Our tool handles all extracted ASTs from source code and processes them through filtering, labeling, and storing stages.
% All these stages also provide extension points to easy use for new tasks.
% \toolname usage is simple as possible, all configuration done by simple YAML file.

We also publish \javanorm, a dataset similar to the popular \emph{Java-small} one: \url{https://doi.org/10.5281/zenodo.6366599}. Compared to \emph{Java-small}, the validation and testing parts of \javanorm contain diverse projects making the evaluation more robust and representative.
The usage of \javanorm does not require additional computational resources, as it has roughly the same size as \emph{Java-small}, yet it allows more robust comparison between models.

All in all, data preprocessing is one of the critical steps when applying machine learning algorithms.
When working with structural representations of source code (\eg in the form of an AST), data preprocessing becomes rather complex and requires the usage of parsers or other external tools.
To make such studies reproducible while maximizing the achieved quality, it is important to properly select a parsing tool and document the selection process in the reports.
We hope that future researchers will take our findings into consideration and will provide more detailed information about the data preparation process in their works.


==> FSE’22_ Parsers evaluation/sections/99-astminer-old.tex <==
\section{\toolname extension}\label{sec:internals}

% \secpart{Overview}
% Use this command to easily switch between proper subsections and simple bold text (which can help to save some space before the deadline).

% \secpart{Extending \toolname}
% Some elaborate description

\secpart{Base for a new tool}
The purpose of this study is to launch a variety of parsers and compare the quality of training on the received data. To achieve this, we needed to run many parsers in a similar pipeline. We could use standalone scripts for each step, but this would lead to significant duplication of code for each parser.

To solve this problem, PathMiner \cite{kovalenko2019pathminer} was taken as the basis of the new tool -- \toolname.

PathMiner is a tool for mining AST, filtering and saving it in some format, originally in bag of paths. Since then support for other formats was added, such as json lines, CSV and DOT. 

Main advantage of PathMiner, that it provides a lot of reusable components. By using PathMiner we could reuse storing algorithms, overall parsing interface and launching architecture.

\secpart{New parsers integration}
Adding new parsers to our \toolname extension is accompanied by the creation of a number of specific objects, which are then built into the general work pipeline. Here we describe how we added those parsers, which comes in form of third-party Java libraries.

Let's see how to add a new parser using the Javaparser example.

To begin with, we need to add a `` wrapper '' inherited from \texttt{Parser} (Figure \ref{fig:jp-parser}), which will serve as an adapter between \toolname and a third-party library. It is also necessary to add a new type of nodes inherited from the abstract class \texttt{Node} to store the resulting tree. Such a division allows to take only the necessary information from a third-party tree, while having the ability to store arbitrary data in the vertices themselves. This can be useful if the structural properties of the tree are still being delegated to other objects.

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/JavaParserNode.pdf}
    \centering
    \caption{Javaparser adapter and new node class}
    \label{fig:jp-parser}
\end{figure}

Further, if we want to train the model using methods from the code (which is true for our case), then we must also implement the \texttt{TreeFunctionSplitter} interface (Figure \ref{fig:jp-splitter}). This is where our instrument starts to diverge from the original. In our extension, the new mandatory interface is \texttt{FunctionInfo} which will collect and store information about the method in a language agnostic way, where the splitter is only searching for methods. Thus, the responsibility for splitting and collecting info about function is split into two entities. Also useful is the fact that it is not necessary to implement the finding of all the information, it is enough to implement only the one that is necessary for a specific task. In our case, we need \texttt{name}, \texttt{modifiers}, \texttt {annotations}, \texttt{isConstructor} . 

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/JavaParserFunctionSplitter.pdf}
    \centering
    \caption{Classes responsible for method search and function info collection.}
    \label{fig:jp-splitter}
\end{figure}

The implementation of these fields unfortunately depends on the grammar, so one must be written for each parser and language. An example of such an implementation can be seen in Listing \ref{lstng:jp_modifiers}

\begin{lstlisting}[
basicstyle=\footnotesize, 
language=Kotlin,
label={lstng:jp_modifiers},
caption={An example of implementation of the \texttt{modifiers} field for \texttt{JavaParserFunctionInfo}}
]
override val modifiers: List<String>? = run {
    // Search for modifiers
    root.children
        .filter { it.typeLabel == MODIFIER }
        .map {
            // For every modifier get it's name
            val token = it.token
            // If no name can be found
            // whole extraction fails
            // meaning that algorithm 
            // doesn't work properly
            if (token == null) { return@run null }
            return@map token
        }
}
\end{lstlisting}

Finally, to bundle all the components together, we need to create new \texttt{ParsingResult} and \texttt{ParsingResultFactory} (Figure \ref{fig:jp-factory}).

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/JavaParserParsingResult.pdf}
    \centering
    \caption{}
    \label{fig:jp-factory}
\end{figure}

By repeating these standard steps for each added instrument and covering the added functionality with tests, we were able to increase the number of instruments in \toolname from 2 to 5.

\secpart{Support for parsers written in other languages}

Since PathMiner was written in Kotlin, it was easy to add support for Java and Kotlin third-party parsers. However, we couldn't add tools written in other languages so easily, which greatly reduced the number of possible parsers for comparison. In \toolname we present new entity \texttt{ForeignParser}. It inherits from \texttt{Parser} and can launch tools from other languages and convert their output to inner tree structure by deserealizing json (Figure \ref{fig:foreign-parser}).

\begin{figure}[h]
\centering
    \includegraphics[width=0.8\columnwidth]{figures/JsonLines.pdf}
    \centering
    \caption{}
    \label{fig:foreign-parser}
\end{figure}

Thus, the task is reduced to writing a wrapper not inside the Astminer tool in the Kotlin language, but inside any other language. This idea can be continued further, for example, having a parser in one language and a utility for converting trees from a native format to json in another. This allows us to extend our tool to all possible parsers that can be run as a separate process with console output.

With this new functionality, we were able to add two more parsers: Tree-sitter and Javalang, by wrapping them in python packages and calling them from \toolname. Listing \ref{lstng:foreign-parser} shows how this looks like in the code of the program itself.

\begin{lstlisting}[basicstyle=\footnotesize, 
language={Kotlin},
caption={Example of supporting javalang -- tool fully written in Python. \texttt{JavaLangParser} can be used as any other parser by calling \texttt{parse} method. \texttt{aw\_javalang} stands for our python wrapper package (hence the name ''aw'' -- additional wrapper) which takes filename as an argument and returns file tree in json format},
label={lstng:foreign-parser}
]
class JavaLangParser : ForeignParser() {
    // Filled for better logging
    override val parser = ParserType.JavaLang
    override val language = FileExtension.Java

    override fun getArguments(file: File) = 
        listOf("aw_javalang", "-f", file.path)
}
\end{lstlisting}

\secpart{AST traceability}
During processing, not all files will go through the parsing stage. The files may contain errors or syntax structures not supported by a particular parser. In such cases, an exception is thrown, the file name is written to the logs, the file itself is skipped and the entire processing continues.

In the case of our research, it is critical that the set of functions on which our model is trained remains unchanged, because the only independent variable we want to present is tree structure obrained from parser output. However, different parsers will produce a different set of functions on the same data. To solve this problem, it is necessary to find some invariant among all trees by which it will then be possible to unambiguously associate each function with its set of trees from different tools. Then all functions that cannot be processed by at least one parser are filtered out. Thus, at the end we will have several datasets with different tree structures, but the same set of methods.

One of these invariants will be the name of the methods and the path to the file that contains it. Unfortunately, although this allowed us to distinguish between many methods, it could not help if several functions have the same name and are in the same file, which, as we learned, is a common practice in the Java language. Thus, these invariants form some groups of methods, from which it is then necessary to take only one (also using some kind of invariant). Initially, we took the smallest tree in terms of the number of vertices, but this is not a strict invariant and does not give a perfect match. Also, by taking only one function from the entire group, the size of the dataset is reduced (up to 10\% of methods are removed from the dataset).

Another approach would be to find invariants in the trees themselves. So, for example, we could define an enclosing element in which the method in question is nested. By enclosing element, we mean Enum, Class or, for example, another function.

Unfortunately, this method, although it gives some results, reducing data loss to 7\%, turned out to be too unstable and very difficult to maintain for each parser.

The final solution turned out to be simple and quite effective. For each function, we will save its position in the code, or rather the beginning and end in row and column format. This information is also not a pure invariant, since the information is provided by the currently used tool, but it is much more stable and reduces data loss to almost zero.

We decided to go a little further and save positions for each vertex and support this functionality for each parser: for those that were already in PathMiner and were integrated by us. We believe this will be useful for future work that associates elements from trees with elements from code and uses this information for analysis or training.

\secpart{Tree normalization}
% trees are huge both in terms of size and depth
% this happens for example because of annotation parsing
% many models filtering trees by size, or cutting trees down (losing info)
% Because of that tree compression algorithm was added
% Compress every consecutive nodes that has 1 child into one node.
 % Type labels will be concatenated with `TOKEN_DELIMITER`.
 % If node with non-empty token will be compressed, new node with
 % the same token will be created to avoid information loss.
 
%   When we experimented with trees obtained using different parsers, we noticed that some tools generate very large trees with long branches, where each vertex has only one child. It was h

As we experimented with the resulting trees, we noticed that some parsers generate trees with long "bamboo" branches. More formally: in trees there are sequences of length $N$ ($N > 3$) from vertices $\{v\}_{1}^{N}$, where the vertex $v_i$ is a descendant of $v_{i-1}$, and at the same time the only one. Such sequences, for example, are often encountered when parsing method and variable declarations. Obviously, the extensive presence of such patterns in trees greatly increases their size. And since modern models try not to train on large trees, just dropping or cutting them by size or depth criteria from the training data, this leads to a smaller training data set and makes some parsers obviously worse than others.

Also, one of the sources of information loss is the fact that in the trees generated by the tools we use, non-leaf vertices can also contain tokens, although this situation is impossible in the definition of AST. For example, when parsing annotations, each package will be represented by a separate vertex, and the package name will be contained as a token. Since the models are designed to work with real abstract syntax trees, tokens in such vertices will not be taken into account in training, which will lead to information loss.

To give odds to such parsers, we applied a single normalization algorithm to all trees before saving them in the required format. Thus, we get trees that are closest to the definition of abstract syntactic.

The algorithm works in 2 steps

\begin{enumerate}
    \item For each non-leaf vertex v that has a non-empty token, create a new child w. Then write a new token v.token to w and replace the token in v with an empty token.
    \item Enter an equivalence relation on the vertices: vertices are equivalent if they belong to the same bamboo branch. Then, for each equivalence class, "connect" the resulting vertices into one, inheriting parameters from the vertices class as follows:
    \begin{lstlisting}[basicstyle=\footnotesize]
def get_new_vertice(class):
    new_v = Node()
    new_v.token = with_max_depth(class).token
    new_v.nodetype = nodetypes(class).join('|')
    new_v.parent = with_min_depth(class).parent
    new_v.children = with_max_depth(class).children
    return new_v
    \end{lstlisting}
\end{enumerate}


==> FSE’22_ Parsers evaluation/sections/99-eval-desc-old.tex <==
% \section{Evaluation description}\label{sec:evaluation}

% \Cref{fig:example-figure} shows that usage of pdf or svg (vector) is preferred over png (raster).

% \begin{figure}[htbp]
% \centering
%     \includegraphics[width=\columnwidth]{figures/example-figure.pdf}
%     \centering
%     \caption{Here goes caption}
%     \label{fig:example-figure}
% \end{figure}

% This section describes how we used the developed \toolname tool for data preprocessing, what we learned about the resulting trees and what results we got in the end.

% \secpart{Preprocessing}
% \textbf{Launch.} After assembling a dataset from projects, we launched astminer using all integrated parsers to generate 8 datasets from trees.

% In the configuration we used, all empty functions (functions without a single line of code) and abstract functions (since obviously they will not contribute to the training of the model) were filtered. In addition to the obvious filtering, we also filtered out constructors in which the method name is not necessarily reflected in the semantics of the method itself, but rather in its environment from other methods and fields.

% Finally, we also filtered out methods with the \texttt {@Override} annotation. The use of such methods can introduce some bias, since, unlike methods with the same name, but outside of a specific class, a method with \texttt{@Override} annotation has a strict context (the body of the class and superclasses) inaccessible to the model during training. In other words, these methods cannot be used for training, since their semantics are not independent and, as a result, are insufficient to predict the name of the method.

% Also, for all 8 parsers, the tree compression feature was used, which we described in the Tool section.

% \textbf {Intersection}. As mentioned earlier, it is necessary that the set of methods on which our model is trained be the same, regardless of the parser. For this, we introduced a new property \texttt{range} for each vertex, which we described in the \ref{} section. Next, we describe how we used it in post-processing data.

% For each dataset, the so-called indexes were built in the form of a table, where each line contained the name of the method, the path to the file containing it and the position of the tree root. Further, it seems obvious to join the indices using the \texttt{join} operation, however, the information about the ranges is provided by the parser itself and, as we learned, is not always accurate. Moreover, different parsers understand the concept of function position differently. So, for example, javaparser includes documentation in the range of a function, while someTool only considers executable code.

% We solved this problem by considering functions to be equal only if their ranges overlap with each other.

% As it turned out, this does not completely solve our problem, since we cannot distinguish extreme cases, such as a method named A inside an anonymous class, which is created in a method named A. However, such situations are very rare and make up no more than 0.002\% of all methods.

% Next, we find all the functions that can be processed by all parsers: these will be functions with 8 trees with intersecting ranges. We call these functions `` good ''. Having received the final indices, we go through all the datasets and collect trees corresponding to good functions.

% \textbf{Embeddings}
% \todo{Ask Egor}

% \secpart{Tree statistic}
% After receiving the datasets, we decided to collect statistics from all trees using structural metrics. This will allow us to form hypotheses and notice some correlation between the results obtained and the structure of the trees.

% In the following pages we show the distributions we got. The metrics we use are: tree size , depth, and average number of children at non-leafed vertices (branching factor).

% \begin{figure}[h]
% \centering
%     \includegraphics[width=\columnwidth]{figures/tree_size.pdf}
%     \centering
%     \caption{Distribution of the tree size}
%     \label{fig:tree-size}
% \end{figure}

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
%  Tool & Min & Max & Mean & Median  \\ \hline
%  ANTLR & 12 & 23,688 & 124.18 & 62 \\ 
%  javaparser & 4 & 10,770 & 58.37 & 30 \\ 
%  JDT & 4 & 10,680 & 63.39 & 34 \\ 
%  javalang & 3 & 15,041 & 79.25 & 40 \\ 
%  PsiMiner & 17 & 33,894 & 191.66 & 103  \\ 
%  Spoon & 4 & 51,920 & 250.66 & 120 \\ 
%  srcML & 5 & 17,629 & 91.60 & 46 \\ 
%  Tree-sitter & 13 & 23,186 & 125.58 & 65 \\ \hline
% \end{tabular}
% \end{table}

% \begin{figure}[h]
% \centering
%     \includegraphics[width=\columnwidth]{figures/tree_depth.pdf}
%     \centering
%     \caption{Distribution of the tree depth}
%     \label{fig:tree-depth}
% \end{figure}

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
%  Tool & Min & Max & Mean & Median  \\ \hline
%  ANTLR & 4 & 291 & 9.74 & 9 \\ 
%  javaparser & 2 & 290 & 7.10 & 7 \\ 
%  JDT & 2 & 542 & 7.93 & 7 \\ 
%  javalang & 2 & 291 & 8.97 & 9 \\ 
%  PsiMiner & 4 & 546 & 10.90 & 10  \\ 
%  Spoon & 2 & 292 & 9.96 & 9 \\ 
%  srcML & 2 & 89 & 9.94 & 10 \\ 
%  Tree-sitter & 4 & 292 & 9.15 & 9 \\ \hline
% \end{tabular}
% \end{table}

% \begin{figure}[h]
% \centering
%     \includegraphics[width=\columnwidth]{figures/bf.pdf}
%     \centering
%     \caption{Distribution of the branching factor}
%     \label{fig:bf}
% \end{figure}

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
%  Tool & Min & Max & Mean & Median  \\ \hline
%  ANTLR & 2.32 & 548.74 & 3.12 & 3.06 \\ 
%  javaparser & 1.64 & 434.5 & 2.69 & 2.5 \\ 
%  JDT & 1.62 & 542 & 2.64 & 2.43 \\ 
%  javalang & 1.57 & 274.95 & 2.27 & 2.19 \\ 
%  PsiMiner & 2.12 & 20.75 & 2.70 & 2.66  \\ 
%  Spoon & 1.75 & 124.70 & 2.40 & 2.4 \\ 
%  srcML & 1.67 & 240.76 & 2.30 & 2.18 \\ 
%  Tree-sitter & 2.36 & 579.28 & 3.23 & 3.20 \\ \hline
% \end{tabular}
% \end{table}


==> FSE’22_ Parsers evaluation/sections/99-motivation-old.tex <==
% When trying to laucnh program we need ast in compilers
% When writing: source code analysis in ide
% When finished we can use AST to search for duplicates

Using a tree structure when manipulating source code is not a new idea. In fact, this approach accompanies the entire development process: from writing the code itself to maintaining it. For example, when using any modern development environment (IDE), built-in code analysis tools are able to infer types, quickly find errors, highlight misused constructs, and find duplicate code. This analysis is possible thanks to parsers that constantly go through the written code and build and update the program model in tree form. 

Then, to compile the program, the compiler builds a model in the form of an AST, checks for all errors, and optimizes parts of the code using built-in heuristics.

Today abstract syntax trees are also increasingly used to evaluate the quality of code. Parsers build trees for the entire project, look for certain patterns, and then, using some criteria, give a final assessment of the project's maintainability.

In general, code analysis using trees has proven to be a more useful practice than using regular expressions, as it allows you to find more complex patterns, and, given the development in this direction, the resulting analysis pipeline does not turn out to be cumbersome and difficult to change.

\secpart{Role of parsers in ML4SE}
Reasearches uses trees to train models by applying convolutions or getting paths
Interesting fact - any tree structure is fine (tree lstm as an example)
People are using some standalone tools that derived from community tools

Recent research shows that machine learning models can gain more information using abstract syntax trees during training. For example, researchers can apply tree convolution, generate paths, collect metrics, and so on. This allows you to improve the result in such tasks as method name prediction, comment generation, code cloning prediction, malware detection and other tasks.

The first step in the above approaches is to get abstract syntax trees. An important note is the fact that there is no single standard or format for them. For training, it is enough to get any tree structure with text labels at each vertex. Moreover, for example, the Tree LSTM model was originally applied to AST obtained from natural language text, and then was reused and adapted for training on source code. This gives a lot of scope for choosing a specific tree structure for training.

Most often, researchers use tree structures from the tools described in the previous section, however, for example, you can use source code trees enriched with additional tags using the IDE. Or you can use raw parse trees, in which the information about the grouping of elements remained in the vertices themselves. Any of this tree structures can be easily built and checked for machine learning application, since most often models do not analyze trees for correctness.


==> FSE’22_ Parsers evaluation/tables/bootstrap-code2seq.tex <==
\begin{tabular}{l|rrrrrrrr}
\textbf{} &
  \multicolumn{1}{l}{\textbf{JDT}} &
  \multicolumn{1}{l}{\textbf{JavaLang}} &
  \multicolumn{1}{l}{\textbf{Tree-Sitter}} &
  \multicolumn{1}{l}{\textbf{JavaParser}} &
  \multicolumn{1}{l}{\textbf{SrcML}} &
  \multicolumn{1}{l}{\textbf{ANTLR}} &
  \multicolumn{1}{l}{\textbf{PSI}} &
  \multicolumn{1}{l}{\textbf{Spoon}} \\ \hline
\textbf{JDT} &
  \multicolumn{1}{l}{-} &
  0.60724 &
  0.73632 &
  0.794 &
  0.8804 &
  0.94456 &
  0.8746 &
  1 \\
\textbf{JavaLang} &
  0.39276 &
  \multicolumn{1}{l}{-} &
  0.66496 &
  0.74488 &
  0.859 &
  0.94648 &
  0.84452 &
  1 \\
\textbf{Tree-Sitter} &
  0.26368 &
  0.33504 &
  \multicolumn{1}{l}{-} &
  0.46392 &
  0.58576 &
  0.61768 &
  0.6742 &
  1 \\
\textbf{JavaParser} &
  0.206 &
  0.25512 &
  0.53608 &
  \multicolumn{1}{l}{-} &
  0.62772 &
  0.6468 &
  0.67348 &
  1 \\
\textbf{SrcML} &
  0.1196 &
  0.141 &
  0.41424 &
  0.37228 &
  \multicolumn{1}{l}{-} &
  0.53228 &
  0.55696 &
  1 \\
\textbf{ANTLR} &
  0.05544 &
  0.05352 &
  0.38232 &
  0.3532 &
  0.46772 &
  \multicolumn{1}{l}{-} &
  0.48276 &
  1 \\
\textbf{PSI} &
  0.1254 &
  0.15548 &
  0.3258 &
  0.32652 &
  0.44304 &
  0.51724 &
  \multicolumn{1}{l}{-} &
  1 \\
\textbf{Spoon} &
  0 &
  0 &
  0 &
  0 &
  0 &
  0 &
  0 &
  \multicolumn{1}{l}{-}
\end{tabular}

==> FSE’22_ Parsers evaluation/tables/bootstrap-treelstm.tex <==
\begin{tabular}{l|rrrrrrrr}
\textbf{} &
  \multicolumn{1}{l}{\textbf{JavaParser}} &
  \multicolumn{1}{l}{\textbf{ANTLR}} &
  \multicolumn{1}{l}{\textbf{JavaLang}} &
  \multicolumn{1}{l}{\textbf{SrcML}} &
  \multicolumn{1}{l}{\textbf{JDT}} &
  \multicolumn{1}{l}{\textbf{Tree-Sitter}} &
  \multicolumn{1}{l}{\textbf{PSI}} &
  \multicolumn{1}{l}{\textbf{Spoon}} \\ \hline
\textbf{JavaParser} &
  \multicolumn{1}{l}{-} &
  0.72404 &
  0.8 &
  0.80008 &
  0.80052 &
  0.86192 &
  0.89024 &
  1 \\
\textbf{ANTLR} &
  0.27596 &
  \multicolumn{1}{l}{-} &
  0.628 &
  0.68052 &
  0.60848 &
  0.69228 &
  0.78752 &
  1 \\
\textbf{JavaLang} &
  0.2 &
  0.372 &
  \multicolumn{1}{l}{-} &
  0.69592 &
  0.54704 &
  0.6354 &
  0.75724 &
  1 \\
\textbf{SrcML} &
  0.19992 &
  0.31948 &
  0.30408 &
  \multicolumn{1}{l}{-} &
  0.45436 &
  0.4078 &
  0.63968 &
  1 \\
\textbf{JDT} &
  0.19948 &
  0.39152 &
  0.45296 &
  0.54564 &
  \multicolumn{1}{l}{-} &
  0.5492 &
  0.74132 &
  1 \\
\textbf{Tree-Sitter} &
  0.13808 &
  0.30772 &
  0.3646 &
  0.5922 &
  0.4508 &
  \multicolumn{1}{l}{-} &
  0.67288 &
  1 \\
\textbf{PSI} &
  0.10976 &
  0.21248 &
  0.24276 &
  0.36032 &
  0.25868 &
  0.32712 &
  \multicolumn{1}{l}{-} &
  0.88 \\
\textbf{Spoon} &
  0 &
  0 &
  0 &
  0 &
  0 &
  0 &
  0.12 &
  \multicolumn{1}{l}{-}
\end{tabular}

==> FSE’22_ Parsers evaluation/tables/model-results.tex <==
%% local settings
\sisetup{detect-weight,mode=text}
% for avoiding siunitx using bold extended
\renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
\renewrobustcmd{\boldmath}{}
% abbreviation
\newrobustcmd{\B}{\bfseries}

\begin{tabular}{l|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Parser}} &
    \multicolumn{4}{c|}{\textbf{TreeLSTM}} &
    \multicolumn{4}{c}{\textbf{Code2Seq}} \\

{} & \textbf{Prec} & \textbf{Rec} & \textbf{F1} & \textbf{ChrF} &
     \textbf{Prec} & \textbf{Rec} & \textbf{F1} & \textbf{ChrF} \\

\hline
\textbf{ANTLR} & $36.0 \pm 1.9$ & $25.5 \pm 1.1$  & $29.8 \pm 1.3$ & $24.8 \pm 1.4$ & $50.2 \pm 1.1$ & $32.7 \pm 0.7$ & $39.6 \pm 0.4$ & $31.3 \pm 0.6$ \\
\textbf{JDT}   & $35.9 \pm 2.2$ & $24.5 \pm 1.3$ & $29.1 \pm 1.6$ & $25.0 \pm 1.2$ & \textbf{51.0 $\pm$ 0.6} & \textbf{33.4 $\pm$ 0.5} & \textbf{40.3 $\pm$ 0.3} & $32.0 \pm 0.4$ \\
\textbf{JavaLang} & $36.4 \pm 1.9$ & $24.7 \pm 1.0$  & $29.4 \pm 1.0$ & $25.1 \pm 1.3$  & $50.7 \pm 0.8$ & $33.1 \pm 0.5$  & $40.0 \pm 0.1$    & $31.9 \pm 0.4$ \\
\textbf{JavaParser} & \textbf{38.2 $\pm$ 2.0} & \textbf{26.0 $\pm$ 1.4} & \textbf{30.9 $\pm$ 1.6} & \textbf{25.7 $\pm$ 1.8} & $49.7 \pm 0.9$ & $33.3 \pm 0.3$ & $39.9 \pm 0.3$  & \textbf{32.2 $\pm$ 0.1} \\
\textbf{PSI} & $35.6 \pm 3.7$ & $22.9 \pm 1.7$ & $27.8 \pm 2.3$ & $23.3 \pm 1.3$  & $50.3 \pm 0.6$  & $32.9 \pm 0.5$  & $39.8 \pm 0.4$ & $31.7 \pm 0.3$ \\
\textbf{Spoon} & $31.6 \pm 1.9$ & $19.9 \pm 1.7$  & $24.3 \pm 1.8$ & $19.6 \pm 1.2$ & $50.1 \pm 0.8$ & $30.9 \pm 0.5$ & $38.2 \pm 0.5$ & $29.8 \pm 0.3$ \\
\textbf{SrcML} & $36.1 \pm 1.9$  & $24.1 \pm 2.0$ & $28.9 \pm 2.0$ & $24.3 \pm 1.8$ & $50.3 \pm 0.9$ & $32.7 \pm 0.4$ & $39.7 \pm 0.5$ & $31.5 \pm 0.2$ \\
\textbf{Tree-Sitter} & $36.4 \pm 1.4$ & $24.1 \pm 1.0$ & $29.0 \pm 1.1$ & $24.0 \pm 0.3$ & $50.4 \pm 0.5$ & $32.4 \pm 0.4$ & $39.4 \pm 0.4$ & $31.1 \pm 0.4$ \\
% \textbf{ANTLR} & $35.98 \pm 1.88$ & $25.5 \pm 1.11$  & $29.84 \pm 1.26$ & $24.77 \pm 1.43$ & $50.23 \pm 1.14$ & $32.73 \pm 0.65$ & $39.62 \pm 0.36$ & $31.28 \pm 0.55$ \\
% \textbf{JDT}   & $35.85 \pm 2.16$ & $24.52 \pm 1.26$ & $29.12 \pm 1.56$ & $24.99 \pm 1.19$ & \textbf{50.95 $\pm$ 0.61} & \textbf{33.39 $\pm$ 0.52} & \textbf{40.34 $\pm$ 0.29} & $31.98 \pm 0.37$ \\
% \textbf{JavaLang} & $36.43 \pm 1.85$ & $24.7 \pm 0.95$  & $29.42 \pm 0.97$ & $25.1 \pm 1.28$  & $50.66 \pm 0.77$ & $33.06 \pm 0.5$  & $40 \pm 0.13$    & $31.87 \pm 0.36$ \\
% \textbf{JavaParser} & \textbf{38.16 $\pm$ 2.03} & \textbf{25.98 $\pm$ 1.43} & \textbf{30.91 $\pm$ 1.56} & \textbf{25.73 $\pm$ 1.84} & $49.71 \pm 0.87$ & $33.34 \pm 0.26$ & $39.91 \pm 0.3$  & \textbf{32.21 $\pm$ 0.14} \\
% \textbf{PSI} & $35.64 \pm 3.68$ & $22.85 \pm 1.66$ & $27.83 \pm 2.33$ & $23.3 \pm 1.32$  & $50.27 \pm 0.6$  & $32.9 \pm 0.45$  & $39.77 \pm 0.36$ & $31.65 \pm 0.32$ \\
% \textbf{Spoon} & $31.62 \pm 1.91$ & $19.78 \pm 1.7$  & $24.33 \pm 1.83$ & $19.58 \pm 1.22$ & $50.07 \pm 0.76$ & $30.92 \pm 0.45$ & $38.23 \pm 0.47$ & $29.79 \pm 0.32$ \\
% \textbf{SrcML} & $36.07 \pm 1.9$  & $24.09 \pm 1.99$ & $28.87 \pm 1.95$ & $24.29 \pm 1.81$ & $50.27 \pm 0.86$ & $32.74 \pm 0.36$ & $39.65 \pm 0.48$ & $31.54 \pm 0.22$ \\
% \textbf{Tree-Sitter} & $36.41 \pm 1.42$ & $24.14 \pm 1.02$ & $29.03 \pm 1.12$ & $24.02 \pm 0.32$ & $50.4 \pm 0.5$   & $32.4 \pm 0.36$  & $39.44 \pm 0.35$ & $31.08 \pm 0.38$ \\
\bottomrule
\end{tabular}

==> FSE’22_ Parsers evaluation/tables/parser-diff.tex <==
\begin{tabular}{l|ccccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Parser}} &
    \multicolumn{5}{c|}{\textbf{Tree metrics (median)}} &
    \textbf{Language} & \textbf{Python} & \textbf{\toolname} \\
& \textbf{TS} & \textbf{TD} & \textbf{BF} & \textbf{UTP} & \textbf{UTK} &
\textbf{support} & \textbf{API} & \textbf{speed (files/sec)}
\\
\hline
\textbf{ANTLR} & 56 & 8 & 3 & 32 & 24 & Any (grammar) & + & 759 \\
\textbf{JDT} & 31 & 6 & 2 & 14 & 19 & Java & - & 1045 \\
\textbf{JavaLang} & 36 & 7 & 2 & 19 & 19 & Java & + & 78 \\
\textbf{JavaParser} & 28 & 6 & 2 & 13 & 17 & Java & - & 938 \\
\textbf{PSI} & 93 & 9 & 2 & 32 & 29 & Any (IntelliJ) & - & 30$^*$ \\
\textbf{Spoon} & 109 & 8 & 2 & 15 & 28 & Java & - & 150 \\
\textbf{SrcML} & 42 & 8 & 2 & 17 & 19 & Java/C/C++/C\# & - & 313 \\
\textbf{Tree-Sitter} & 60 & 8 & 3 & 25 & 27 & Any (grammar) & + & 117 \\
\bottomrule
\end{tabular}

==> FSE’22_ Parsers evaluation/tables/tree-stats.tex <==
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Parser}} &
    \multicolumn{3}{c|}{\textbf{TS}} &
    \multicolumn{3}{c|}{\textbf{D}} &
    \multicolumn{3}{c|}{\textbf{BF}} &
    \multicolumn{3}{c|}{\textbf{UTP}} &
    \multicolumn{3}{c}{\textbf{UTK}} \\
{} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} \\
\hline
\textbf{ANTLR} & 13 & 56 & 353 & 3 & 8 & 16 & 2.8 & 3 & 3.5 & 19 & 32 & 55 & 11 & 24 & 68 \\
\textbf{JDT} & 5 & 31 & 176 & 1 & 6 & 15 & 2 & 2 & 4 & 6 & 14 & 27 & 6 & 19 & 64 \\
\textbf{JavaLang} & 8 & 36 & 220 & 3 & 7 & 15 & 1.9 & 2 & 2.7 & 10 & 19 & 36 & 6 & 19 & 65 \\
\textbf{JavaParser} & 5 & 28 & 162 & 1 & 6 & 12 & 2.1 & 2 & 4 & 7 & 13 & 24 & 6 & 17 & 60 \\
\textbf{PSI} & 22 & 93 & 527 & 4 & 9 & 18 & 2.5 & 2 & 2.9 & 19 & 32 & 54 & 12 & 29 & 86 \\
\textbf{Spoon} & 25 & 109 & 716 & 6 & 8 & 15 & 2.2 & 2 & 2.6 & 10 & 15 & 26 & 10 & 28 & 87 \\
\textbf{SrcML} & 7 & 42 & 260 & 2 & 8 & 17 & 1.9 & 2 & 3 & 9 & 17 & 26 & 6 & 19 & 69 \\
\textbf{Tree-Sitter} & 14 & 60 & 353 & 3 & 8 & 15 & 2.84 & 3 & 3.7 & 14 & 25 & 47 & 12 & 27 & 79 \\
\bottomrule
\end{tabular}

==> FSE’22_ Parsers evaluation/tables/ttest.tex <==
\begin{tabular}{l|cccccccc}
\toprule
{} & \textbf{ANTLR} & \textbf{JDT} & \textbf{JavaLang} & \textbf{JavaParser} & \textbf{PSI} & \textbf{Spoon} & \textbf{SrcML} & \textbf{Tree-Sitter} \\
\hline
\textbf{ANTLR}       & - & - & - & - & UTP & TD & TD & TS \\
\textbf{JDT}         & - & - & TS, UTK & TS, UTK & - & - & UTK & - \\
\textbf{JavaLang}    & - & TS, UTK & - & UTK & - & - & TS, UTK & TD  \\
\textbf{JavaParser}  & - & TS, UTK & UTK & - & BF & - & UTK & - \\
\textbf{PSI}         & UTP & - & - & BF & - & UTK & - & UTK \\
\textbf{Spoon}       & TD & - & - & - & UTK & - & TD & UTK  \\
\textbf{SrcML}       & TD & UTK & TS, UTK & UTK & - & TD & - & - \\
\textbf{Tree-Sitter} & TS & - & TD & - & UTK & UTK & - & - \\
\bottomrule
\end{tabular}

==> sections/99-astminer-old.tex <==
\section{\toolname extension}\label{sec:internals}

% \secpart{Overview}
% Use this command to easily switch between proper subsections and simple bold text (which can help to save some space before the deadline).

% \secpart{Extending \toolname}
% Some elaborate description

\secpart{Base for a new tool}
The purpose of this study is to launch a variety of parsers and compare the quality of training on the received data. To achieve this, we needed to run many parsers in a similar pipeline. We could use standalone scripts for each step, but this would lead to significant duplication of code for each parser.

To solve this problem, PathMiner \cite{kovalenko2019pathminer} was taken as the basis of the new tool -- \toolname.

PathMiner is a tool for mining AST, filtering and saving it in some format, originally in bag of paths. Since then support for other formats was added, such as json lines, CSV and DOT. 

Main advantage of PathMiner, that it provides a lot of reusable components. By using PathMiner we could reuse storing algorithms, overall parsing interface and launching architecture.

\secpart{New parsers integration}
Adding new parsers to our \toolname extension is accompanied by the creation of a number of specific objects, which are then built into the general work pipeline. Here we describe how we added those parsers, which comes in form of third-party Java libraries.

Let's see how to add a new parser using the Javaparser example.

To begin with, we need to add a `` wrapper '' inherited from \texttt{Parser} (Figure \ref{fig:jp-parser}), which will serve as an adapter between \toolname and a third-party library. It is also necessary to add a new type of nodes inherited from the abstract class \texttt{Node} to store the resulting tree. Such a division allows to take only the necessary information from a third-party tree, while having the ability to store arbitrary data in the vertices themselves. This can be useful if the structural properties of the tree are still being delegated to other objects.

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/JavaParserNode.pdf}
    \centering
    \caption{Javaparser adapter and new node class}
    \label{fig:jp-parser}
\end{figure}

Further, if we want to train the model using methods from the code (which is true for our case), then we must also implement the \texttt{TreeFunctionSplitter} interface (Figure \ref{fig:jp-splitter}). This is where our instrument starts to diverge from the original. In our extension, the new mandatory interface is \texttt{FunctionInfo} which will collect and store information about the method in a language agnostic way, where the splitter is only searching for methods. Thus, the responsibility for splitting and collecting info about function is split into two entities. Also useful is the fact that it is not necessary to implement the finding of all the information, it is enough to implement only the one that is necessary for a specific task. In our case, we need \texttt{name}, \texttt{modifiers}, \texttt {annotations}, \texttt{isConstructor} . 

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/JavaParserFunctionSplitter.pdf}
    \centering
    \caption{Classes responsible for method search and function info collection.}
    \label{fig:jp-splitter}
\end{figure}

The implementation of these fields unfortunately depends on the grammar, so one must be written for each parser and language. An example of such an implementation can be seen in Listing \ref{lstng:jp_modifiers}

\begin{lstlisting}[
basicstyle=\footnotesize, 
language=Kotlin,
label={lstng:jp_modifiers},
caption={An example of implementation of the \texttt{modifiers} field for \texttt{JavaParserFunctionInfo}}
]
override val modifiers: List<String>? = run {
    // Search for modifiers
    root.children
        .filter { it.typeLabel == MODIFIER }
        .map {
            // For every modifier get it's name
            val token = it.token
            // If no name can be found
            // whole extraction fails
            // meaning that algorithm 
            // doesn't work properly
            if (token == null) { return@run null }
            return@map token
        }
}
\end{lstlisting}

Finally, to bundle all the components together, we need to create new \texttt{ParsingResult} and \texttt{ParsingResultFactory} (Figure \ref{fig:jp-factory}).

\begin{figure}[h]
\centering
    \includegraphics[width=\columnwidth]{figures/JavaParserParsingResult.pdf}
    \centering
    \caption{}
    \label{fig:jp-factory}
\end{figure}

By repeating these standard steps for each added instrument and covering the added functionality with tests, we were able to increase the number of instruments in \toolname from 2 to 5.

\secpart{Support for parsers written in other languages}

Since PathMiner was written in Kotlin, it was easy to add support for Java and Kotlin third-party parsers. However, we couldn't add tools written in other languages so easily, which greatly reduced the number of possible parsers for comparison. In \toolname we present new entity \texttt{ForeignParser}. It inherits from \texttt{Parser} and can launch tools from other languages and convert their output to inner tree structure by deserealizing json (Figure \ref{fig:foreign-parser}).

\begin{figure}[h]
\centering
    \includegraphics[width=0.8\columnwidth]{figures/JsonLines.pdf}
    \centering
    \caption{}
    \label{fig:foreign-parser}
\end{figure}

Thus, the task is reduced to writing a wrapper not inside the Astminer tool in the Kotlin language, but inside any other language. This idea can be continued further, for example, having a parser in one language and a utility for converting trees from a native format to json in another. This allows us to extend our tool to all possible parsers that can be run as a separate process with console output.

With this new functionality, we were able to add two more parsers: Tree-sitter and Javalang, by wrapping them in python packages and calling them from \toolname. Listing \ref{lstng:foreign-parser} shows how this looks like in the code of the program itself.

\begin{lstlisting}[basicstyle=\footnotesize, 
language={Kotlin},
caption={Example of supporting javalang -- tool fully written in Python. \texttt{JavaLangParser} can be used as any other parser by calling \texttt{parse} method. \texttt{aw\_javalang} stands for our python wrapper package (hence the name ''aw'' -- additional wrapper) which takes filename as an argument and returns file tree in json format},
label={lstng:foreign-parser}
]
class JavaLangParser : ForeignParser() {
    // Filled for better logging
    override val parser = ParserType.JavaLang
    override val language = FileExtension.Java

    override fun getArguments(file: File) = 
        listOf("aw_javalang", "-f", file.path)
}
\end{lstlisting}

\secpart{AST traceability}
During processing, not all files will go through the parsing stage. The files may contain errors or syntax structures not supported by a particular parser. In such cases, an exception is thrown, the file name is written to the logs, the file itself is skipped and the entire processing continues.

In the case of our research, it is critical that the set of functions on which our model is trained remains unchanged, because the only independent variable we want to present is tree structure obrained from parser output. However, different parsers will produce a different set of functions on the same data. To solve this problem, it is necessary to find some invariant among all trees by which it will then be possible to unambiguously associate each function with its set of trees from different tools. Then all functions that cannot be processed by at least one parser are filtered out. Thus, at the end we will have several datasets with different tree structures, but the same set of methods.

One of these invariants will be the name of the methods and the path to the file that contains it. Unfortunately, although this allowed us to distinguish between many methods, it could not help if several functions have the same name and are in the same file, which, as we learned, is a common practice in the Java language. Thus, these invariants form some groups of methods, from which it is then necessary to take only one (also using some kind of invariant). Initially, we took the smallest tree in terms of the number of vertices, but this is not a strict invariant and does not give a perfect match. Also, by taking only one function from the entire group, the size of the dataset is reduced (up to 10\% of methods are removed from the dataset).

Another approach would be to find invariants in the trees themselves. So, for example, we could define an enclosing element in which the method in question is nested. By enclosing element, we mean Enum, Class or, for example, another function.

Unfortunately, this method, although it gives some results, reducing data loss to 7\%, turned out to be too unstable and very difficult to maintain for each parser.

The final solution turned out to be simple and quite effective. For each function, we will save its position in the code, or rather the beginning and end in row and column format. This information is also not a pure invariant, since the information is provided by the currently used tool, but it is much more stable and reduces data loss to almost zero.

We decided to go a little further and save positions for each vertex and support this functionality for each parser: for those that were already in PathMiner and were integrated by us. We believe this will be useful for future work that associates elements from trees with elements from code and uses this information for analysis or training.

\secpart{Tree normalization}
% trees are huge both in terms of size and depth
% this happens for example because of annotation parsing
% many models filtering trees by size, or cutting trees down (losing info)
% Because of that tree compression algorithm was added
% Compress every consecutive nodes that has 1 child into one node.
 % Type labels will be concatenated with `TOKEN_DELIMITER`.
 % If node with non-empty token will be compressed, new node with
 % the same token will be created to avoid information loss.
 
%   When we experimented with trees obtained using different parsers, we noticed that some tools generate very large trees with long branches, where each vertex has only one child. It was h

As we experimented with the resulting trees, we noticed that some parsers generate trees with long "bamboo" branches. More formally: in trees there are sequences of length $N$ ($N > 3$) from vertices $\{v\}_{1}^{N}$, where the vertex $v_i$ is a descendant of $v_{i-1}$, and at the same time the only one. Such sequences, for example, are often encountered when parsing method and variable declarations. Obviously, the extensive presence of such patterns in trees greatly increases their size. And since modern models try not to train on large trees, just dropping or cutting them by size or depth criteria from the training data, this leads to a smaller training data set and makes some parsers obviously worse than others.

Also, one of the sources of information loss is the fact that in the trees generated by the tools we use, non-leaf vertices can also contain tokens, although this situation is impossible in the definition of AST. For example, when parsing annotations, each package will be represented by a separate vertex, and the package name will be contained as a token. Since the models are designed to work with real abstract syntax trees, tokens in such vertices will not be taken into account in training, which will lead to information loss.

To give odds to such parsers, we applied a single normalization algorithm to all trees before saving them in the required format. Thus, we get trees that are closest to the definition of abstract syntactic.

The algorithm works in 2 steps

\begin{enumerate}
    \item For each non-leaf vertex v that has a non-empty token, create a new child w. Then write a new token v.token to w and replace the token in v with an empty token.
    \item Enter an equivalence relation on the vertices: vertices are equivalent if they belong to the same bamboo branch. Then, for each equivalence class, "connect" the resulting vertices into one, inheriting parameters from the vertices class as follows:
    \begin{lstlisting}[basicstyle=\footnotesize]
def get_new_vertice(class):
    new_v = Node()
    new_v.token = with_max_depth(class).token
    new_v.nodetype = nodetypes(class).join('|')
    new_v.parent = with_min_depth(class).parent
    new_v.children = with_max_depth(class).children
    return new_v
    \end{lstlisting}
\end{enumerate}


==> sections/99-eval-desc-old.tex <==
% \section{Evaluation description}\label{sec:evaluation}

% \Cref{fig:example-figure} shows that usage of pdf or svg (vector) is preferred over png (raster).

% \begin{figure}[htbp]
% \centering
%     \includegraphics[width=\columnwidth]{figures/example-figure.pdf}
%     \centering
%     \caption{Here goes caption}
%     \label{fig:example-figure}
% \end{figure}

% This section describes how we used the developed \toolname tool for data preprocessing, what we learned about the resulting trees and what results we got in the end.

% \secpart{Preprocessing}
% \textbf{Launch.} After assembling a dataset from projects, we launched astminer using all integrated parsers to generate 8 datasets from trees.

% In the configuration we used, all empty functions (functions without a single line of code) and abstract functions (since obviously they will not contribute to the training of the model) were filtered. In addition to the obvious filtering, we also filtered out constructors in which the method name is not necessarily reflected in the semantics of the method itself, but rather in its environment from other methods and fields.

% Finally, we also filtered out methods with the \texttt {@Override} annotation. The use of such methods can introduce some bias, since, unlike methods with the same name, but outside of a specific class, a method with \texttt{@Override} annotation has a strict context (the body of the class and superclasses) inaccessible to the model during training. In other words, these methods cannot be used for training, since their semantics are not independent and, as a result, are insufficient to predict the name of the method.

% Also, for all 8 parsers, the tree compression feature was used, which we described in the Tool section.

% \textbf {Intersection}. As mentioned earlier, it is necessary that the set of methods on which our model is trained be the same, regardless of the parser. For this, we introduced a new property \texttt{range} for each vertex, which we described in the \ref{} section. Next, we describe how we used it in post-processing data.

% For each dataset, the so-called indexes were built in the form of a table, where each line contained the name of the method, the path to the file containing it and the position of the tree root. Further, it seems obvious to join the indices using the \texttt{join} operation, however, the information about the ranges is provided by the parser itself and, as we learned, is not always accurate. Moreover, different parsers understand the concept of function position differently. So, for example, javaparser includes documentation in the range of a function, while someTool only considers executable code.

% We solved this problem by considering functions to be equal only if their ranges overlap with each other.

% As it turned out, this does not completely solve our problem, since we cannot distinguish extreme cases, such as a method named A inside an anonymous class, which is created in a method named A. However, such situations are very rare and make up no more than 0.002\% of all methods.

% Next, we find all the functions that can be processed by all parsers: these will be functions with 8 trees with intersecting ranges. We call these functions `` good ''. Having received the final indices, we go through all the datasets and collect trees corresponding to good functions.

% \textbf{Embeddings}
% \todo{Ask Egor}

% \secpart{Tree statistic}
% After receiving the datasets, we decided to collect statistics from all trees using structural metrics. This will allow us to form hypotheses and notice some correlation between the results obtained and the structure of the trees.

% In the following pages we show the distributions we got. The metrics we use are: tree size , depth, and average number of children at non-leafed vertices (branching factor).

% \begin{figure}[h]
% \centering
%     \includegraphics[width=\columnwidth]{figures/tree_size.pdf}
%     \centering
%     \caption{Distribution of the tree size}
%     \label{fig:tree-size}
% \end{figure}

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
%  Tool & Min & Max & Mean & Median  \\ \hline
%  ANTLR & 12 & 23,688 & 124.18 & 62 \\ 
%  javaparser & 4 & 10,770 & 58.37 & 30 \\ 
%  JDT & 4 & 10,680 & 63.39 & 34 \\ 
%  javalang & 3 & 15,041 & 79.25 & 40 \\ 
%  PsiMiner & 17 & 33,894 & 191.66 & 103  \\ 
%  Spoon & 4 & 51,920 & 250.66 & 120 \\ 
%  srcML & 5 & 17,629 & 91.60 & 46 \\ 
%  Tree-sitter & 13 & 23,186 & 125.58 & 65 \\ \hline
% \end{tabular}
% \end{table}

% \begin{figure}[h]
% \centering
%     \includegraphics[width=\columnwidth]{figures/tree_depth.pdf}
%     \centering
%     \caption{Distribution of the tree depth}
%     \label{fig:tree-depth}
% \end{figure}

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
%  Tool & Min & Max & Mean & Median  \\ \hline
%  ANTLR & 4 & 291 & 9.74 & 9 \\ 
%  javaparser & 2 & 290 & 7.10 & 7 \\ 
%  JDT & 2 & 542 & 7.93 & 7 \\ 
%  javalang & 2 & 291 & 8.97 & 9 \\ 
%  PsiMiner & 4 & 546 & 10.90 & 10  \\ 
%  Spoon & 2 & 292 & 9.96 & 9 \\ 
%  srcML & 2 & 89 & 9.94 & 10 \\ 
%  Tree-sitter & 4 & 292 & 9.15 & 9 \\ \hline
% \end{tabular}
% \end{table}

% \begin{figure}[h]
% \centering
%     \includegraphics[width=\columnwidth]{figures/bf.pdf}
%     \centering
%     \caption{Distribution of the branching factor}
%     \label{fig:bf}
% \end{figure}

% \begin{table}[h]
% \centering
% \begin{tabular}{lccccc}
% \hline
%  Tool & Min & Max & Mean & Median  \\ \hline
%  ANTLR & 2.32 & 548.74 & 3.12 & 3.06 \\ 
%  javaparser & 1.64 & 434.5 & 2.69 & 2.5 \\ 
%  JDT & 1.62 & 542 & 2.64 & 2.43 \\ 
%  javalang & 1.57 & 274.95 & 2.27 & 2.19 \\ 
%  PsiMiner & 2.12 & 20.75 & 2.70 & 2.66  \\ 
%  Spoon & 1.75 & 124.70 & 2.40 & 2.4 \\ 
%  srcML & 1.67 & 240.76 & 2.30 & 2.18 \\ 
%  Tree-sitter & 2.36 & 579.28 & 3.23 & 3.20 \\ \hline
% \end{tabular}
% \end{table}


==> sections/99-motivation-old.tex <==
% When trying to laucnh program we need ast in compilers
% When writing: source code analysis in ide
% When finished we can use AST to search for duplicates

Using a tree structure when manipulating source code is not a new idea. In fact, this approach accompanies the entire development process: from writing the code itself to maintaining it. For example, when using any modern development environment (IDE), built-in code analysis tools are able to infer types, quickly find errors, highlight misused constructs, and find duplicate code. This analysis is possible thanks to parsers that constantly go through the written code and build and update the program model in tree form. 

Then, to compile the program, the compiler builds a model in the form of an AST, checks for all errors, and optimizes parts of the code using built-in heuristics.

Today abstract syntax trees are also increasingly used to evaluate the quality of code. Parsers build trees for the entire project, look for certain patterns, and then, using some criteria, give a final assessment of the project's maintainability.

In general, code analysis using trees has proven to be a more useful practice than using regular expressions, as it allows you to find more complex patterns, and, given the development in this direction, the resulting analysis pipeline does not turn out to be cumbersome and difficult to change.

\secpart{Role of parsers in ML4SE}
Reasearches uses trees to train models by applying convolutions or getting paths
Interesting fact - any tree structure is fine (tree lstm as an example)
People are using some standalone tools that derived from community tools

Recent research shows that machine learning models can gain more information using abstract syntax trees during training. For example, researchers can apply tree convolution, generate paths, collect metrics, and so on. This allows you to improve the result in such tasks as method name prediction, comment generation, code cloning prediction, malware detection and other tasks.

The first step in the above approaches is to get abstract syntax trees. An important note is the fact that there is no single standard or format for them. For training, it is enough to get any tree structure with text labels at each vertex. Moreover, for example, the Tree LSTM model was originally applied to AST obtained from natural language text, and then was reused and adapted for training on source code. This gives a lot of scope for choosing a specific tree structure for training.

Most often, researchers use tree structures from the tools described in the previous section, however, for example, you can use source code trees enriched with additional tags using the IDE. Or you can use raw parse trees, in which the information about the grouping of elements remained in the vertices themselves. Any of this tree structures can be easily built and checked for machine learning application, since most often models do not analyze trees for correctness.


==> tables/bootstrap-code2seq.tex <==
\begin{tabular}{l|rrrrrrrr}
\textbf{} &
  \multicolumn{1}{l}{\textbf{JDT}} &
  \multicolumn{1}{l}{\textbf{JavaLang}} &
  \multicolumn{1}{l}{\textbf{Tree-Sitter}} &
  \multicolumn{1}{l}{\textbf{JavaParser}} &
  \multicolumn{1}{l}{\textbf{SrcML}} &
  \multicolumn{1}{l}{\textbf{ANTLR}} &
  \multicolumn{1}{l}{\textbf{PSI}} &
  \multicolumn{1}{l}{\textbf{Spoon}} \\ \hline
\textbf{JDT} &
  \multicolumn{1}{l}{-} &
  0.60724 &
  0.73632 &
  0.794 &
  0.8804 &
  0.94456 &
  0.8746 &
  1 \\
\textbf{JavaLang} &
  0.39276 &
  \multicolumn{1}{l}{-} &
  0.66496 &
  0.74488 &
  0.859 &
  0.94648 &
  0.84452 &
  1 \\
\textbf{Tree-Sitter} &
  0.26368 &
  0.33504 &
  \multicolumn{1}{l}{-} &
  0.46392 &
  0.58576 &
  0.61768 &
  0.6742 &
  1 \\
\textbf{JavaParser} &
  0.206 &
  0.25512 &
  0.53608 &
  \multicolumn{1}{l}{-} &
  0.62772 &
  0.6468 &
  0.67348 &
  1 \\
\textbf{SrcML} &
  0.1196 &
  0.141 &
  0.41424 &
  0.37228 &
  \multicolumn{1}{l}{-} &
  0.53228 &
  0.55696 &
  1 \\
\textbf{ANTLR} &
  0.05544 &
  0.05352 &
  0.38232 &
  0.3532 &
  0.46772 &
  \multicolumn{1}{l}{-} &
  0.48276 &
  1 \\
\textbf{PSI} &
  0.1254 &
  0.15548 &
  0.3258 &
  0.32652 &
  0.44304 &
  0.51724 &
  \multicolumn{1}{l}{-} &
  1 \\
\textbf{Spoon} &
  0 &
  0 &
  0 &
  0 &
  0 &
  0 &
  0 &
  \multicolumn{1}{l}{-}
\end{tabular}

==> tables/bootstrap-treelstm.tex <==
\begin{tabular}{l|rrrrrrrr}
\textbf{} &
  \multicolumn{1}{l}{\textbf{JavaParser}} &
  \multicolumn{1}{l}{\textbf{ANTLR}} &
  \multicolumn{1}{l}{\textbf{JavaLang}} &
  \multicolumn{1}{l}{\textbf{SrcML}} &
  \multicolumn{1}{l}{\textbf{JDT}} &
  \multicolumn{1}{l}{\textbf{Tree-Sitter}} &
  \multicolumn{1}{l}{\textbf{PSI}} &
  \multicolumn{1}{l}{\textbf{Spoon}} \\ \hline
\textbf{JavaParser} &
  \multicolumn{1}{l}{-} &
  0.72404 &
  0.8 &
  0.80008 &
  0.80052 &
  0.86192 &
  0.89024 &
  1 \\
\textbf{ANTLR} &
  0.27596 &
  \multicolumn{1}{l}{-} &
  0.628 &
  0.68052 &
  0.60848 &
  0.69228 &
  0.78752 &
  1 \\
\textbf{JavaLang} &
  0.2 &
  0.372 &
  \multicolumn{1}{l}{-} &
  0.69592 &
  0.54704 &
  0.6354 &
  0.75724 &
  1 \\
\textbf{SrcML} &
  0.19992 &
  0.31948 &
  0.30408 &
  \multicolumn{1}{l}{-} &
  0.45436 &
  0.4078 &
  0.63968 &
  1 \\
\textbf{JDT} &
  0.19948 &
  0.39152 &
  0.45296 &
  0.54564 &
  \multicolumn{1}{l}{-} &
  0.5492 &
  0.74132 &
  1 \\
\textbf{Tree-Sitter} &
  0.13808 &
  0.30772 &
  0.3646 &
  0.5922 &
  0.4508 &
  \multicolumn{1}{l}{-} &
  0.67288 &
  1 \\
\textbf{PSI} &
  0.10976 &
  0.21248 &
  0.24276 &
  0.36032 &
  0.25868 &
  0.32712 &
  \multicolumn{1}{l}{-} &
  0.88 \\
\textbf{Spoon} &
  0 &
  0 &
  0 &
  0 &
  0 &
  0 &
  0.12 &
  \multicolumn{1}{l}{-}
\end{tabular}

==> tables/tree-stats.tex <==
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Parser}} &
    \multicolumn{3}{c|}{\textbf{TS}} &
    \multicolumn{3}{c|}{\textbf{D}} &
    \multicolumn{3}{c|}{\textbf{BF}} &
    \multicolumn{3}{c|}{\textbf{UTP}} &
    \multicolumn{3}{c}{\textbf{UTK}} \\
{} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} & \textbf{5th} & \textbf{50th} & \textbf{95th} \\
\hline
\textbf{ANTLR} & 13 & 56 & 353 & 3 & 8 & 16 & 2.8 & 3 & 3.5 & 19 & 32 & 55 & 11 & 24 & 68 \\
\textbf{JDT} & 5 & 31 & 176 & 1 & 6 & 15 & 2 & 2 & 4 & 6 & 14 & 27 & 6 & 19 & 64 \\
\textbf{JavaLang} & 8 & 36 & 220 & 3 & 7 & 15 & 1.9 & 2 & 2.7 & 10 & 19 & 36 & 6 & 19 & 65 \\
\textbf{JavaParser} & 5 & 28 & 162 & 1 & 6 & 12 & 2.1 & 2 & 4 & 7 & 13 & 24 & 6 & 17 & 60 \\
\textbf{PSI} & 22 & 93 & 527 & 4 & 9 & 18 & 2.5 & 2 & 2.9 & 19 & 32 & 54 & 12 & 29 & 86 \\
\textbf{Spoon} & 25 & 109 & 716 & 6 & 8 & 15 & 2.2 & 2 & 2.6 & 10 & 15 & 26 & 10 & 28 & 87 \\
\textbf{SrcML} & 7 & 42 & 260 & 2 & 8 & 17 & 1.9 & 2 & 3 & 9 & 17 & 26 & 6 & 19 & 69 \\
\textbf{Tree-Sitter} & 14 & 60 & 353 & 3 & 8 & 15 & 2.84 & 3 & 3.7 & 14 & 25 & 47 & 12 & 27 & 79 \\
\bottomrule
\end{tabular}
